BBB-Voting: 1-out-of-k Blockchain-Based Boardroom Voting

Voting is a means to agree on a collective decision based on available choices (e.g., candidates), where participants agree to abide by their outcome. To improve some features of e-voting, decentralized blockchain-based solutions can be employed, where the blockchain represents a public bulletin board that in contrast to a centralized bulletin board provides extremely high availability, censorship resistance, and correct code execution. A blockchain ensures that all entities in the voting system have the same view of the actions made by others due to its immutability and append-only features. The existing remote blockchain-based boardroom voting solution called Open Voting Network (OVN) provides the privacy of votes, universal & End-to-End verifiability, and perfect ballot secrecy; however, it supports only two choices and lacks robustness enabling recovery from stalling participants. We present BBB-Voting, an equivalent blockchain-based approach for decentralized voting such as OVN, but in contrast to it, BBB-Voting supports 1-out-of-$k$ choices and provides robustness that enables recovery from stalling participants. We make a cost-optimized implementation using an Ethereum-based environment respecting Ethereum Enterprise Alliance standards, which we compare with OVN and show that our work decreases the costs for voters by 13.5% in normalized gas consumption. Finally, we show how BBB-Voting can be extended to support the number of participants limited only by the expenses paid by the authority and the computing power to obtain the tally.

==> sec/abstract.tex <==
Voting is a means to agree on a collective decision based on available choices (e.g., candidates), where participants (voters) agree to abide by their outcome. 
To improve some features of e-voting, decentralized solutions based on a blockchain can be employed, where the blockchain represents a public bulletin board that in contrast to a centralized bulletin board provides $100\%$ availability and censorship resistance.
A blockchain ensures that all entities in the voting system have the same view of the actions made by others due to its immutable and append-only log. 
The existing blockchain-based boardroom voting solution called Open Voting Network (OVN) provides the privacy of votes and perfect ballot secrecy, but it supports only two choices. 
We present \name, an equivalent blockchain-based approach for decentralized voting such as OVN, but in contrast to it, \name supports 1-out-of-$k$ choices and provides a fault tolerance mechanism that enables recovery from stalling participants. 
%We resolve the problem of stalling participants by a fault recovery protocol.
We provide a cost-optimized implementation using Ethereum, which we compare with OVN and show that our work decreases the costs for voters by $13.5\%$ in terms of gas consumption.
%Next, we outline that our implementation scaling  is twice as high w.r.t number of participants in a boardroom voting, while preserving the costs paid by the authority and participants -- we made proof-of-concept experiments with up to 100 participants.

  
%Finally, fault tolerance, a major limitation of OVN is resolved in our boardroom voting -- when a voter is not available to execute the fault recovery step, then her vote is also removed from the tally, without restarting the protocol. \ih{too detailed. The reader has no chance to understand it here.} 
%Such a scenario and solution is presented in Khader et al.~\cite{KhaderSRH12}, and we rely on it for the fault recovery presented. \ih{this is detail and should be rather in the text.}
 
%\keywords{Boardroom Voting  $\bullet$ Blockchain  $\bullet$ Self-Tallying Protocol $\bullet$ Fault Tolerance $\bullet$ Ethereum.}

==> sec/analysis.tex <==

%\subsection{Efficiency of finding candidate vote count}
%\subsection{Time Complexity to Decode Tally}
%\label{ssec:compefficiency}

%A tally is encoded in the multiplication of all blinded votes $\prod\limits_{i=1}^{n}B_i$ and it can be encoded by exhaustive search over various vote counts. 
%The complexity of reconstructing the tally results (see \autoref{eqn:eq3}) is bounded by ${n+k-1}\choose{k}$ combinations with repetitions ($n$ participants and $k$ choices). \ih{duplicate info.}
%Fewer enumeration attempts allow us to efficiently reconstruct the candidate results from the tally \ih{is tally different than candidate results? \textbf{Sarad}.. yes, tally is just the multiplication of blinded votes. Next, the number of votes each candidate received needs to be recovered from tally} and is a goal of the tally computation.
%We provide an upper bound on the number of attempts required for decoding the tally in \autoref{}.
%In the brute force solution, we also check $k!$ permutations for each combination, subject to the constraint $\sum\limits_{i=1}^{k} ct_i = n $.
%The maximum number of brute force attempts is
%${n+k-1}\choose{k}$.
%From this bound, we observe the size of $k$ (candidates) is dominant in our ability to decode the tally in comparison to $n$ (participants).
%In practice, when $k\ll n$ it is within the realm of feasible computations.
%If $n=50,k=8$, the maximum brute force attempts is $\approx 2^{30.6}$.
%For example, if $n=100 \wedge k=6$, the maximum number of attempts is $ \approx 2^{30.5}$, and it is trivial to compute.
%At $n=200,k=4$, it is $\approx 2^{26}$.
%In the case of a referendum, where $k=2$, there is only ${n+2-1}\choose{1}$ combinations to brute force.
%Hence, it is trivial to decode the tally for even larger number of participants in a booth.
%The time required to brute force a 40 bit symmetric key~\cite{fortybitenc2019} may serve as a baseline on the ease of brute forcing up to $2^{40}$ operations.
%\autoref{table:bruteforceattempts} gives the upper bound on enumeration attempts required to recover individual candidate results per booth.



%\setlength{\tabcolsep}{4pt}
%\begin{table}
%	\footnotesize
%	\centering
%	\begin{tabular}{@{}rllr@{}}
%		
%		\toprule
%		\textbf{Component}   & \textbf{Language}           & \textbf{Techonology} & \textbf{LoC} \\
%		\Xhline{1\arrayrulewidth} \noalign{\smallskip}
%		Voting Smart Contract       & Solidity, Javascript        & Truffle              & 647          \\
%		Aggregation Smart Contract       & Solidity, Javascript        & Truffle              & 647          \\
%		Authority 		     & Javascript         		& -- 	&1939         \\
%		Voter 		     & Javascript         		& -- 	&1939         \\
%		Tests                & Javascript                  & Truffle              & 1166         \\
%		\Xhline{1\arrayrulewidth} \noalign{\smallskip}
%		\textbf{Sum}         &                             &                      & 5316         \\ \bottomrule
%	\end{tabular}
%	\caption{Development effort in Lines of Code (LoC). \IH{TODO}}	
%	\label{tab:loc}
%	%		\vspace{0.3cm}
%	
%\end{table}




==> sec/blockchain-and-centralized-voting.tex <==
In this section, we compare blockchain  e-voting with centralized e-voting since blockchain e-voting has received some critique~\cite{critic-blockchain-for-voting,park2021going} in the past. 
We use \name as an in-line example and we conclude that blockchain voting can only improve the potential problems of centralized voting at the cost of more complex governance.

\myparagraph{\textbf{Bulletin Board vs. Blockchains}} 
The definition of a bulletin board~\cite{Kiayias2002} assumes its immutability and append-only feature.
While the bulletin board is a conceptual data structure, its expected behavior is not possible to perfectly guarantee neither in centralized voting nor blockchain voting.
However, in centralized voting, a single entity can decide about removing/modifying an entry in the bulleting board, while in blockchain voting such a decision has to be made by a quorum of the honest majority. 
Hence, the blockchain intuitively provides stronger append-only and immutability guarantees.

\myparagraph{\textbf{Device Exploitation at Participants}} 
Park et al.~\cite{park2021going} discuss several categories of attacks on electronic voting systems.
The first of them is \textit{device exploitation}, in which $\mathcal{A}$ tampers with the hardware or software of $P$s, and thus she can change cast vote for the malicious one -- we argue that this attack is the same in both centralized and blockchain voting, and it depends on the protections made at the $P$'s side.
To thwart such attacks, signing of the vote should be done in a dedicated tamper resistance device (i.e., hardware security module (HSM)), which stores the private keys of $P$, while the device must contain a display capable of presenting the data being signed to $P$.
Although such devices might be used in both types of voting, they are more common in the blockchain scenario, where they are referred to as \textit{hardware wallets} (e.g., Trezor, Ledger, KeepKey).
We refer the reader to the work of Arapinis et al.~\cite{ArapinisGKK19} for the security analysis of hardware wallets, where the authors emphasize the importance of ``see-what-you-sign'' on a display of a HW wallet to thwart tampering. % at the clients.
%Note that signing the vote on a secure standalone device and moving the vote to a networked device ensures that any malware on the latter is unable to correctly sign a bogus vote. \ih{it is implicit}
%\footnote{On the other hand, a disadvantage of hardware wallets is their high cost (\$100-\$150), which might be a problem for large scale voting.} 
%

\myparagraph{\textbf{Device Exploitation at Voting System}}
Another option for a device exploitation is compromising the voting system itself (i.e., its infrastructure).
In the case of centralized voting, the difficulty (and also the cost) of compromising a single centralized e-voting system  is lower than compromising a majority of consensus nodes\footnote{I.e., nodes with a majority of consensus power.} in a decentralized infrastructure of blockchain.
Park et al.~\cite{park2021going} state that device exploitation within e-voting infrastructure may prevent voters from casting their votes as intended (and thus violating E2E verifiability~\cite{benaloh2015end}). % and let them believe they did cast the votes.
%
%However, it is clear that there is no difference in device exploitation of the client between both voting types.
We argue that while there is no difference in device exploitation of the client between both voting types, centralized voting is significantly more vulnerable to censorship and availability attacks when device exploitation occurs on its centralized infrastructure, as opposed to decentralized blockchain voting that provides extremely high availability (see also below).


\myparagraph{\textbf{(D)DoS Attacks}}
The authority of centralized voting is exposed to a potential (D)DoS attack during the whole period of running.
In contrast, $VA$ in \name is exposed to a potential DoS attack only during the registration phase while the remaining phases run under high availability (depending on a particular blockchain).

\myparagraph{\textbf{Censorship}}
Blockchain voting improves the censorship resistance problem of centralized voting -- intuitively, it is more likely that the vote censorship will be perpetrated due to a decision made by a single entity in centralized voting than the majority of consensus power in the blockchain.

Josh Benaloh went further and put the censorship into the position for the conflict-of-interest~\cite{critic-blockchain-for-voting}: ``\textit{Suppose the transactions are votes, and I am the leader of a movement to oppose a heavy tax on blockchain miners. If I am going to vote in that referendum, then I have to convince some blockchain miner to pick up my vote and put it into the chain.}''
%
We argue that in the case of suspicion on a conflict-of-interest, the most convenient blockchain platform can be selected for the voting protocol (i.e., \name) since each protocol run is independent.
%We assume that Benaloh refers to a (public) permissionless blockchain with Proof-of-Work (PoW) consensus protocol (such as Bitcoin) with miners.
%However, we argue that such a blockchain type is not suitable for voting.
%\sarad{do we need to say this, we use public ethereum. pls refer to slack discussion.}
%
Moreover, running \name over a public permissionless blockchain might be too expensive for particular use cases, such as large-scale elections. % (due to transaction fees).
For such use cases, more suitable types are permissioned or semi-permissioned~\cite{sra-survey} blockchains running a Proof-of-Stake and/or BFT consensus protocols (see \autoref{ssec:cost-perf-limitations}). 
%
Nevertheless, in any type of blockchain,  multiple consensus nodes substitute a part of functionalities provided by a single authority in centralized voting, which improves the censorship resistance.\footnote{Note that identity verification and registration can remain centralized, as might be requested by organizers of large-scale elections.}
%

Finally, a single honest consensus node is sufficient to provide the public with indisputable proof of vote censorship perpetrated by a dishonest majority if it occurs -- such a proof would contain a valid block including a censored transaction, which was produced by an honest node but was abandoned in an orphaned fork by the dishonest majority. 
Furthermore, a hash of such a block might be timestamped by a secure timestamping service to provide proof that the block existed in the time of fork occurrence  (e.g., OpenTimestamps, POEX.IO, STAMPD).
%(e.g., OpenTimestamps,\footnote{\url{https://opentimestamps.org/}} POEX.IO,\footnote{\url{https://poex.io/}} STAMPD,\footnote{\url{https://stampd.io/}} Bitcoin.com Notary\footnote{\url{https://notary.bitcoin.com/}}) to prove the existence of the block at the time the fork occurred.
This is not possible in centralized voting since voting authority can contend the voter had not cast her vote. 

%\ih{Park et al.~\cite{park2021going} mentions the fees payed }

\myparagraph{\textbf{Lost Private Keys}}
Park et al.~\cite{park2021going} state that $P$s who lose their blockchain keys are unable to vote and recovery of the key in is not possible, as opposed to centralized voting.
We argue that \name (and blockchain voting in general) is a one-time short process ranging from a few hours to a few days during which $P$s generate a new key-pair for interaction with the blockchain as well as a new ephemeral key-pair for homomorphic encryption.
Hence, the probability of losing a newly generated key in such a short time is very low.


\myparagraph{\textbf{Coercion and Vote Selling}}
When comparing centralized voting with block\-chain voting, the coercion and vote-selling problems remain the same -- both are possible due to the remote location of voting, while the blockchain does not bring any disadvantages in contrast to centralized voting.
%Vote selling is possible since blinded votes are recorded in the public bulleting board in both cases.
Besides, the coercion resistance (and thus receipt-freeness), which is in general attributed to local voting systems, is not guaranteed in these systems if trusted $VA$ misbehaves and involves in it~\cite{chaum2008scantegrity}.


\myparagraph{\textbf{Data Feeds}}
Park et al.~\cite{park2021going} emphasize issues of decentralized data feeds (a.k.a., oracles) such as Augur~\cite{peterson2015augur}, ChainLink~\cite{ellisdecentralized}, Witnet~\cite{de2017witnet}.
However, we argue that the blockchain voting does not require any data feed service and can run on a smart contract platform using solely the data submitted by $VA$ and $P$s.

\myparagraph{\textbf{Fixing Bugs}}
Park et al.~\cite{park2021going} criticize additional complexity and required coordination related to fixing bugs across the infrastructure of blockchains in contrast to centralized voting. 
However, this is considered a tax for decentralization and other beneficial blockchain features. 
Nevertheless, such coordination is manageable in all blockchain types and is usually defined in the governance model.

==> sec/conclusion.tex <==
In this paper, we proposed \name, a 1-out-of-$k$ blockchain-based boardroom voting solution that supports fault tolerance. 
%We also supplied the necessary cryptographic primitives to provide verifiability for all steps in the election.
%The ZKP of set membership was updated to reflect the number of choices.
%A simple fault recovery protocol is also presented, so the tally is not stalled.
%Blockchain smart contracts were invoked to act as a tamper-resistant and  non-equivocal log for carrying out the steps in the voting protocol.
%It served to reduce the need to trust individuals.
%Scalability in design and implementation resulted in decentralized voting to scale from a boardroom voting to tens of thousands of participants.
%Analysis showed the protocol supported the security and privacy requirements, and was practical.
%Implementation optimizations saw costs reduce by nearly 24\% when compared with the latest work in this direction. 
%Building on our scalable and more cost-efficient voting protocol, a corrective governance protocol to maintain accountability was proposed.
%Finally, extended support for fault tolerance and receipt-indistinguishability was provided.
%We further aim to investigate game theoretic efficiencies in incentivizing participants through a smart contract treasury to remain engaged in corrective governance and update our scheme into a post quantum secure cryptographic protocol. 
%However, a quantum computing attack is not expected to constitute an immediate threat to public key cryptography~\cite{Schneier2018}. 
We made two variants of full implementation on the Ethereum -- one based on elliptic curve DLP and the other one based on DLP for integer modulo $p$.
We showed that only the elliptic curve variant is feasible in the real settings of public blockchains.
We performed several cost optimizations and discussed further improvements concerning costs and scalability, where we made a proof-of-concept implementation with up to 1000 voters.
Finally, we compared our solution with OVN and results indicate that \name reduces the costs for voters and the authority by $13.5\%$ and $0.9\%$, respectively; while additionally offering robustness.
%To conclude, OVN supports nearly 50 participants and \name supports 135 participants.
%OVN support 2 candidates and \name is suitable for 2 or more candidates. 
%The costs of \name are reduced in contrast to OVN due to a few optimizations that we proposed in \autoref{ssec:optimizatations}.
%However, we note that caching in MPC key computation was also utilized in OVN.

%\ih{Among optimizations, we modify the blinded vote verification~\cite{Kiayias2002} into its equivalent form enabling us to optimize multiplication on elliptic curves by w-NAF~\cite{hankerson2005guide} scalar decomposition.}


==> sec/discussion-new.tex <==
\vspace{-0.3cm}
In this section, we discuss the extensions addressing the scalability and performance limitations of \name. 
%We also discuss other possible cost and performance optimizations and their security trade-off.

\vspace{-0.2cm}
%\myparagraph{\textbf{Scalability Limitations \& Extension}}
\subsection{Scalability Limitation \& Extension}
\label{ssec:scalability-improvements}
\vspace{-0.2cm}
The limitation of \name (like in OVN) is a lack of scalability, where the block gas limit might be exceeded with a high number of $P$s.
Therefore, we primarily position our solution as boardroom voting; however, we will  show in this section that it can be extended even to larger voting.
%
%
Our voting protocol (see \autoref{ssec:basicprotocol}) has a few platform-specific bottlenecks. % that might exceed the block gas limit of Ethereum, when either $k$ or $n$ reach particular values.
The first bottleneck is in the setup phase, where $VA$ submits the wallet addresses of all $P$s to SC in a single transaction, which might exceed the block gas limit when the number of participants $n > 201$.
%However, we have shown that 100 participants per booth is more than a sufficient number to protect them from privacy violations due to booth sharding (see \autoref{ssec:shardinganalysis}). 
The second bottleneck occurs in the pre-voting phase, where $VA$ calls the function of $SC$ to compute all MPC keys; exceeding the block gas limit occurs when the number of participants $n > 135$. % (considerin12g all introduced optimizations).
%This is resolved by batching to allow an arbitrary number of participants in the election.
The next bottleneck occurs in the voting phase, 
where voters submit their blinded votes together with 1-out-of-$k$ ZKP,
exceeding the block gas limit when the number of choices $k > 7$.
The last bottleneck occurs in the fault recovery phase and the block gas limit is exceeded when the number of simultaneously faulty participants $f > 9$.
%To resolve this bottleneck, the ZKP verification in the right side of \autoref{fig:ECCZKPMultiCandidate} can be batched as well.
%In the case of vote submission, we assume that the maximal number of candidates equal to five is sufficient for proof-of-concept.


%
\begin{figure}% {0.62\textwidth}
%	\vspace*{-0.8cm}
	\centering
	\includegraphics[width=0.7\linewidth]{fig/gas/mpc-batches.pdf}
	\caption{A computation of MPC keys by the authority $VA$ using various batch sizes and the most optimized ECC implementation, demonstrating a scalability extension of \name, which also mitigates a privacy issue of unanimous and majority voting.}
	\label{fig:mpc-batches}
%	\vspace*{-0.6cm}
\end{figure}
%
Nevertheless, transaction batching can be introduced for the elimination of all these bottlenecks.
To realize a batching of pre-voting, voting, and fault-recovery  phases, the additional integrity preservation logic across batches needs to be addressed while the verification of integrity has to be made by $SC$.
%
For demonstration purposes, we addressed the bottleneck of the pre-voting stage (see \autoref{fig:mpc-batches})  and setup stage, 
which further improves the vote privacy in \name (see \autoref{sec:blockchain-specific-issues}) and causes only a minimal cost increase due to the overhead of integrity preservation (i.e., 1\%).
With this extension, $n$ is limited only by the expenses paid by $VA$ to register $P$s, compute their MPC keys, and its computing power to obtain the tally.\footnote{E.g., for $n = 1000$, $k=2 ~(\text{and} ~k=4)$, it takes $0.15$s (and $\sim4$h) to obtain the tally on a commodity PC with 8 cores, respectively.}
If a certain combination of high $n$ and $k$ would make computation of a tally overly computationally expensive (or the cost of its verification by $SC$), it is further possible to partition $P$s into multiple groups (i.e., voting booths), each managed by an instance of \name, while the total results could be summed across instances.
Scalability evaluation of such an approach and other operations is subject to our our other work which provides more empirical evidence~\cite{stanvcikova2022sbvote}. % where we will focus on blockchain-based large-scale elections. 





\subsection{Cost and Performance Limitations}\label{ssec:cost-perf-limitations}
\vspace{-0.3cm}
%\myparagraph{\textbf{Further Cost Optimizations}}
Although we thoroughly optimized the costs (and thus performance) of our implementation (see \autoref{ssec:optimizatations}), the expenses imposed by a public permissionless smart contract platform might be still high, especially during peaks of the gas price and/or in the case of a larger voting than boardroom voting (see \autoref{ssec:scalability-improvements}).
Besides, the transactional throughput of such platforms might be too small for such larger voting instances to occur in a specified time window.
Therefore, to further optimize the costs of \name and its performance, it can run on a 
public permissioned Proof-of-Authority platforms, e.g., using Hyperledger projects (such as safety-favored Besu with BFT).
Another option is to use smart contract platforms backed by the trusted computing that off-chains expensive computations (e.g., Ekiden~\cite{cheng2019ekiden}, TeeChain~\cite{lind2019teechain}, Aquareum~\cite{homoliak2020aquareum}), or other partially-decentralized second layer solutions (e.g., Plasma~\cite{plasma-eth}, Polygon Matic~\cite{polygon-matic-investopedia}, Hydra~\cite{chakravarty2020hydra}). 
%\paragraph{\textbf{Timeouts and Deposits.}}
%Although we did not focus on timeouts for each phase of our protocol, we emphasize that timeouts are an important part of the protocol, and we include them in the implementation. 
%Likewise, deposit-based penalties for misbehaving involved parties is also an important aspect of the voting protocol, which should incentivize the voters to vote and the authority to not stall in shifting phases of the protocol.
%If any of the involved parties stalls in the protocol after the expiration of a particular timeout, the value deposited is split among the remaining involved parties. 
Even though these solutions might preserve most of the blockchain features harnessed in e-voting, availability and decentralization might be decreased, which is part of the security/performance trade-off.




==> sec/discussion.tex <==
%\ih{[Move to analysis] Since our voting protocol belongs to the class of protocols outputting the full tally of votes, $\mathcal{A}$ can infer vote choices only in the case of unanimous voting by all participants, which is the natural property of such protocols.)}


First, we compare blockchain  e-voting with centralized e-voting (see \autoref{sec:centralized-vs-blockchain-voting}) since blockchain voting has received some critique~\cite{critic-blockchain-for-voting,park2021going}, and we use \name as an in-line example.
%Note that the discussion about blockchain voting also holds for \name, and we use it as an example.
%Finally, we make a security analysis of e-voting features in \name with respect to ElGamal cryptosystem in \autoref{ssec:security}.


\subsection{\textbf{Centralized vs. Blockchain E-Voting}}\label{sec:centralized-vs-blockchain-voting}
%Centralized solutions seen are not byzantine fault tolerant, where as a blockchain is a byzantine State Machine Replication.
%From hacked single server solutions such as SUNDR~\cite{LiKMS04}, it is evident that detecting user equivocation is possible, only once a user shares the view of her log with the other user holding their own view of the log (\textit{fork-consistency}).
%Where there are many users with full access rights to the server, it may additional be possible that some of the users are adversarial in nature and may equivocate. A byzantine fault tolerant message passing consesnus  will be required for users log to arrive at a consistent state. Solutions such as pBFT~\cite{CastroL99} are known not to scale, and is the reason why other byzantine fault tolerant consensus such as Bitcoin proof-of-work is used.
%In the case of SUNDR, once the number of users are very high (e.g., 100000 users),  each user maintaing her log is required to carry out an excessive amount of message passing and the solution may not scale. 

\myparagraph{\textbf{Bulletin Board vs. Blockchains}}
The definition of a bulletin board from Kiayias and Yung~\cite{Kiayias2002} assumes its immutability and append-only feature.
While the bulletin board is a conceptual data structure, its expected behavior is not possible to perfectly guarantee neither in centralized voting nor blockchain voting.
However, in centralized voting, a single entity can decide about removing/modifying an entry in the bulleting board, while in blockchain voting such a decision has to be made by a quorum of the honest majority. 
Hence, the blockchain intuitively provides stronger append-only and immutability guarantees.


CAP theorem~\cite{brewer2000towards} enables a distributed system (such as the blockchain) to select either \textbf{\underline{c}}onsistency or  \textbf{\underline{a}}vailability during the time of network \textbf{\underline{p}}artitions.
If the system selects consistency (e.g., Algorand~\cite{gilad2017algorand}, BFT-based blockchains such as HyperLedger~\cite{hyperledger1}), it stalls during network partitions and does not provide liveness (i.e., the blocks are not produced) but provides safety (i.e., all nodes agree on the same blocks when some are produced). 
%
If the system selects availability (e.g., Bitcoin~\cite{Satoshi2009}, Ethereum~\cite{wood2014}), it does not provide safety but provides liveness (i.e., it does not stall), which translates into possibility of creating \textit{accidental forks} and eventually accepting one as valid.
%
Many public blockchains favor availability over consistency, and thus do not guarantee immediate immutability. 
%
%These accidental forks occur mainly due to a non-negligible network propagation delay, during which, several consensus nodes (i.e., miners) might produce different valid blocks at the same length, while only one of these blocks will be eventually included in a blockchain.\footnote{The winning block of such a fork contains a ``stronger'' value that meets the requested difficulty in contrast to losing block -- e.g., in Ethereum~\cite{wood2014} or Bitcoin~\cite{Satoshi2009}, where the stronger value of the target is represented by the smaller hash of a header. Note that in other consensus protocols (e.g., Algorand~\cite{gilad2017algorand}, HyperLedger~\cite{hyperledger1}), the notion of ``stronger'' is represented by the number of votes cast by the consensus nodes.} 
%
Furthermore, blockchains might suffer from \textit{malicious forks} that are longer than accidental forks and are expensive for the attacker. 
Usually, their goal is to execute double-spending\footnote{Assuming 51\% / 33\% of malicious nodes in PoW / BFT-based protocols, respectively.} or selfish mining~\cite{eyal2018majority}, violating the assumptions of the consensus protocol employed. % within a blockchain.  
%\footnote{Note that the main goal of the selfish mining is to earn more than the fair ratio of the attacker's consensus power to the consensus power of the whole network; this is possible by letting other consensus nodes to waste their consensus power on building a chain that will be later replaced by a secret malicious chain.} 
%that require $33\%$ of the total consensus power or $51\%$ attacks that violate the assumptions of the consensus protocol employed within a blockchain but are the most expensive to execute. 

To prevent accidental forks and mitigate malicious forks in liveness-favoring blockchains, it is recommended to wait for a certain number of blocks (a.k.a., block confirmations / a time to finality) to increase the probability that a transaction will remain irreversible after it appears in the blockchain. % and thus minimize the probability that the blockchain will be overridden -- such a time interval is referred to as \textit{a time to finality}. 
%For example, in Ethereum, the time to finality is equal to $\sim$3 minutes, which corresponds to 12 block confirmations.
%
Another option to cope with this threat is to utilize consensus protocols that favor safety over liveness (such as~\cite{gilad2017algorand,hyperledger1}), which provide immediate time to finality. % that is more convenient for the e-voting use case. 
%with a fast time to finalities, such as Algorand~\cite{gilad2017algorand}, HoneyBadgerBFT~\cite{miller2016honey}, or StrongChain~\cite{strongchain}. 
%

Considering \name as an example, we argue that these forks are not critical for the proposed protocol since any transaction can be resubmitted if it is not included in the blockchain after a fork.
%
Waiting for the time to finality (with a potential resubmission) can be done as a background task of the client software at $P$s' devices, so $P$s do not have to wait.
%Moreover, if a transaction of the client would not be included due to an accidental fork, the client software can automatically resubmit the transaction.
Finally, we emphasize that the time to finality is negligible in contrast to timeouts of the protocol phases; therefore, there is enough time to make an automatic resubmission if needed.


\myparagraph{\textbf{Device Exploitation at Participants}}
Park et al.~\cite{park2021going} discuss several categories of attacks on electronic voting systems.
The first of them is \textit{device exploitation}, in which the adversary tampers with the hardware or software of $P$s, and thus she can change cast vote for the malicious one -- we argue that this attack is the same in both centralized and blockchain voting, and it depends on the protections made at the $P$'s side.
To thwart such attacks, signing of the vote should be done in a dedicated tamper resistance device (i.e., hardware security module (HSM)), which stores the private keys of the user, while the device must contain a display capable of presenting the data being signed to $P$.
Although such devices might be used in both types of voting, they are more common in the blockchain scenario, where they are referred to as \textit{hardware wallets} (e.g., Trezor, Ledger, KeepKey).
We refer the reader to the work of Arapinis et al.~\cite{ArapinisGKK19} for the security analysis of hardware wallets, where the authors emphasize the importance of ``see-what-you-sign'' on a display of a HW wallet to thwart tampering. % at the clients.
%Note that signing the vote on a secure standalone device and moving the vote to a networked device ensures that any malware on the latter is unable to correctly sign a bogus vote. \ih{it is implicit}
%\footnote{On the other hand, a disadvantage of hardware wallets is their high cost (\$100-\$150), which might be a problem for large scale voting.} 
%

\myparagraph{\textbf{Device Exploitation at Voting System}}
Another option for a device exploitation is compromising the voting system itself (i.e., its infrastructure).
In the case of centralized voting, the difficulty (and also the cost) of compromising a single centralized e-voting system  is lower than compromising a majority of consensus nodes\footnote{I.e., nodes with a majority of consensus power.} in a decentralized infrastructure of blockchain.
Park et al.~\cite{park2021going} state that device exploitation within e-voting infrastructure may prevent voters from casting their votes as intended (and thus violating E2E verifiability~\cite{benaloh2015end}). % and let them believe they did cast the votes.
%
%However, it is clear that there is no difference in device exploitation of the client between both voting types.
We argue that while there is no difference in device exploitation of the client between both voting types, centralized voting is significantly more vulnerable to censorship and availability attacks when device exploitation occurs on its centralized infrastructure, as opposed to decentralized blockchain voting that provides extremely high availability (see also below).


\myparagraph{\textbf{(D)DoS Attacks}}
The authority of centralized voting is moreover exposed to a potential (D)DoS attack during the whole period of running.
In contrast, $VA$ in \name is exposed to a potential DoS attack only during the registration phase while the remaining phases run under high availability (depending on a particular blockchain).

\myparagraph{\textbf{Censorship}}
Blockchain voting improves the censorship resistance problem of centralized voting -- intuitively, it is more likely that the vote censorship will be perpetrated due to a decision made by a single entity in centralized voting than the majority of consensus power in the blockchain.

Josh Benaloh went further and put the censorship into the position for the conflict-of-interest~\cite{critic-blockchain-for-voting}: ``\textit{Suppose the transactions are votes, and I am the leader of a movement to oppose a heavy tax on blockchain miners. If I am going to vote in that referendum, then I have to convince some blockchain miner to pick up my vote and put it into the chain.}''
%
We argue that in the case of suspicion on a conflict-of-interest, the most convenient blockchain platform can be selected for the voting protocol (i.e., \name) since each protocol run is independent.
%We assume that Benaloh refers to a (public) permissionless blockchain with Proof-of-Work (PoW) consensus protocol (such as Bitcoin) with miners.
%However, we argue that such a blockchain type is not suitable for voting.
%\sarad{do we need to say this, we use public ethereum. pls refer to slack discussion.}
%
Moreover, running \name over a public permissionless blockchain might be too expensive for particular use cases, such as large-scale elections. % (due to transaction fees).
For such use cases, more suitable types are permissioned or semi-permissioned~\cite{sra-survey} blockchains running a Proof-of-Stake and/or BFT consensus protocol, 
%
Nevertheless, in any type of blockchain,  multiple consensus nodes substitute a part of functionalities provided by a single authority in centralized voting, which improves the censorship resistance.\footnote{Note that identity verification and registration can remain centralized, as might be requested by organizers of large-scale elections.}
%

Finally, a single honest consensus node is sufficient to provide the public with indisputable proof of vote censorship perpetrated by a dishonest majority if it occurs -- such a proof would contain a valid block including a censored transaction, which was produced by an honest node but was abandoned in an orphaned fork by the dishonest majority. 
Furthermore, a hash of such a block might be timestamped by a secure timestamping service to provide proof that the block existed in the time of fork occurrence  (e.g., OpenTimestamps, POEX.IO, STAMPD).
%(e.g., OpenTimestamps,\footnote{\url{https://opentimestamps.org/}} POEX.IO,\footnote{\url{https://poex.io/}} STAMPD,\footnote{\url{https://stampd.io/}} Bitcoin.com Notary\footnote{\url{https://notary.bitcoin.com/}}) to prove the existence of the block at the time the fork occurred.
This is not possible in centralized voting since voting authority can contend the voter had not cast her vote. 

%\ih{Park et al.~\cite{park2021going} mentions the fees payed }

\myparagraph{\textbf{Lost Private Keys}}
Park et al.~\cite{park2021going} state that participants who lose their blockchain keys are unable to vote and recovery of the key in the blockchain is not possible, as opposed to credentials recovery of centralized voting.
%We argue that other important information is not included in their work.
% and thus they mislead the readers.
We argue that \name (and blockchain voting in general) is a one-time short process ranging from a few hours to a few days during which $P$s generate a new key-pair for interaction with the blockchain as well as a new ephemeral key-pair for homomorphic encryption.
Hence, the probability of losing a newly generated key in such a short time is very low.
%
%Second, if a participant loses her blockchain key after the voting is finished, she might ``re-register'' at $VA$ with a fresh key (i.e., blockchain address) when the next voting takes place.
% -- the registration and identity verification are centralized (e.g., HTTPS service, such as in \name), and thus a participant logs in with her existing credentials.


\myparagraph{\textbf{Coercion and Vote Selling}}
When comparing centralized voting with block\-chain voting, in general, the coercion and vote-selling problems remain the same -- both are possible due to the remote location of voting, while the blockchain does not bring any disadvantages in contrast to centralized voting.
%Vote selling is possible since blinded votes are recorded in the public bulleting board in both cases.

\myparagraph{\textbf{Data Feeds}}
Park et al.~\cite{park2021going} emphasize issues of decentralized data feeds (a.k.a., oracles) such as Augur~\cite{peterson2015augur}, ChainLink~\cite{ellisdecentralized}, Witnet~\cite{de2017witnet}.
However, we argue that the blockchain voting does not require any data feed service and can run on a smart contract platform using solely the data submitted by $VA$ and $P$s.

\myparagraph{\textbf{Fixing Bugs}}
Park et al.~\cite{park2021going} criticize additional complexity and required coordination related to fixing bugs across the infrastructure of blockchains in contrast to centralized voting. 
However, this is considered a tax for decentralization and other beneficial blockchain features. 
Nevertheless, such coordination is manageable in all blockchain types and is usually defined in the governance model.


%PArk: There are simpler, more reliable ways to achieve a public bulletin board, such as traditional database technology.


%All the previous points about the blockchain hold only when one 


%Note that such waiting can be done as a background task of $\mathbb{C}$, hence $\mathbb{U}$ does not have to wait.




%
%In blockchains with a long time to finality, overly fast confirmation of an operation may be dangerous, as, if an operation were initiated in an ``incorrect'' view, an attacker holding $SK_{\mathbb{U}}$ would hijack the OTP and reuse it for a malicious operation settled in the ``correct'' view. 
%
%
% We stress that for our protocol it is crucial to wait such a recommended number of block confirmations before submission of a confirmation transaction, and thus ensure that an initialization transaction cannot be reversed.\footnote{The same applies to the first two stages when introducing a new root hash.}
% Nevertheless, such a waiting can be implemented at the client, hence a user would not have to wait.












==> sec/ftolerance.tex <==
We extend the base variant of \name by a fault recovery mechanism.
If one or more $P$s stall (i.e., are faulty) and do not submit their blinded vote in the voting stage despite committing in doing so, the tally cannot be computed directly.
%We refer to them as \textit{faulty} $P$s.
To recover from faulty $P$s, we adapt the solution proposed by Khader et al.~\cite{KhaderSRH12}, and we place the fault recovery phase immediately after the voting phase. % of our protocol.
All remaining honest $P$s are expected to repair their vote by a transaction to $SC$, which contains key materials shared with all faulty $P$s and their NIZK proof of correctness.
$SC$ verifies all key materials with proofs (see  \autoref{fig:ZKPdiffie}), and then they are used to invert out the counter-party keys from a blinded vote of an honest $P$ who sent the vote-repairing transaction to $SC$.
%


\subsubsection{Faults in Fault Recovery.}
Even if some of the honest (i.e., non-faulty) $P$s would be faulty during the recovery phase (i.e., do not submit vote-repairing transaction), it is still possible to recover from such a state by repeating the next round of the fault recovery, but this time only with key materials related to new faulty $P$s.
Such a partial repair of votes enables us to save costs imposed by the smart contract platform, and thus already submitted key materials need to be neither resubmitted nor verified. % since no restart of the e-voting protocol is required.
As a consequence of the fault recovery, it is not necessary to restart the voting protocol, which substantially increases the resistance of our approach to serious failures.
%
An issue that needs to be addressed in the fault recovery is $\mathcal{A}$ who controls multiple $P$s and let them stall one-by-one in each fault recovery round. 
To disincentivize such a behavior, we require stalling $P$s of each recovery round to lose their deposits, which is split across remaining $P$s as a compensation for the cost of fault recovery -- therefore, the value of the deposit must reflect it.
Moreover, additional (increasing) deposit might be required in each fault-recovery round.



%
%\ih{Drop?} Each pair of $P$s $P_i$ and $P_j$ ($i\neq j$) have their ephemeral public keys $g^{x_i}$ and $g^{x_j}$ published on the blockchain.
%Hence, $P_i$ using her private key $x_i$ can compute $g^{x_ix_j}$ and $P_j$ with her private key $x_j$ can compute  $g^{x_jx_i}$. 
%Thus, each pair of $P$s has their counter-party key material shared.
%%I.e, each pair is able to compute $g^{x_ix_j}$ =  $g^{x_jx_i}$, where each participant in the pair is \textit{counter-party} to the other.
%%If the counter-party is not available to remove a detected faulty $P$s' key material (i.e., all $g^{x_ix_j}$ and their NIZK proofs) -- the counter-party is also treated as faulty and her vote is removed from the tally.
%After all honest $P$s submit the vote-repairing transaction and no new faulty $P$s are detected during a timeout, the state is shifted to the tally phase, where the votes of all faulty $P$s are excluded by $SC$, and already repaired blinded votes are used for verification of \autoref{eqn:eq3}, executed at $SC$.

	

\begin{figure}[t]
	\begin{center}
		\vspace{-0.3cm}
		\fbox{\scriptsize
			\begin{protocolm}{2}	
				
				\participants{\underline{$Participant~P_i$}}{\underline{Smart Contract}}%\\ 						
				\participants{\underline{$A\leftarrow g^{x_i},B
						\leftarrow g^{x_j},x_i$}}{\underline{$A\leftarrow g^{x_i},~B\leftarrow g^{x_j}$}}%\\				
				Let~w_i,\in_{r}\mathbb{F}_p\\
				C\leftarrow g^{x_ix_j}\\
				m_1\leftarrow {g}^{w_i}\\
				m_2\leftarrow {B}^{w_i}  \\ %&&\stackrel{m_1,m_2}{\xrightarrow{\hspace*{0.75cm}}}\\
				
				
				
				c\leftarrow  \Hzk(A,B,m_1,m_2)\\ 	
				r_i\leftarrow w_i+ cx_i &&\\
				&\sends{C,r_i,m_1,m_2} & c\leftarrow  \Hzk(A,B,m_1,m_2)\\			
				%&& &&(From~reconstructed~s_{ij})\\
				
				
				&  & g^r\stackrel{?}{=}{m_1}{A^c}\\
				&  & B^r\stackrel{?}{=}{m_2}{C^c}\\
				
				
			\end{protocolm}
		}
	\end{center}
	\vspace{-0.35cm}
	\caption{ZKP verifying correspondence of $g^{x_ix_j}$ to public keys $A=g^{x_i}, B=g^{x_j}$. 
		%	Participant steps and communication of parameters to the smart contract are carried out as part of the deal phase. The smart contract proceeds with verification in the reconstruction phase, once $s_{ij}=g^{x_ix_j}$ is reconstructed and available to the contract. \ih{too detailed and intuitive}
	}
	\label{fig:ZKPdiffie}
	\vspace{-0.5cm}
\end{figure}



\myparagraph{\textbf{Example}}
\autoref{fig:linear} depicts two faulty participants $P_3$ and $P_5$.
First, we assume that there is one faulty participant $P_3$ after the voting phase.
Therefore, in the execution of the fault recovery round, $P_3$'s key material must be removed from the blinded votes of all other benign $P$s by inverting out their counter-party key materials $\forall P_i \setminus P_3: g^{x_ix_3}$.
In detail, all benign $P$s are supposed to submit a vote repairing transaction to $SC$ to finish the fault recovery.
%
However, say $P_5$ (intentionally) stalls during the fault recovery execution.
%the counter-party of $P_3$ required to remove $g^{x_3x_5}$ (from $P_5$'s blinded vote),
In this case, after the expiration of timeout for fault recovery round, $P_5$ is also treated as faulty, and all remaining participants $\forall P_i \setminus \{P_3, P_5\}$ must re-execute the fault recovery again, this time only with one key material $g^{x_ix_5}$ related to $P_5$ and its NIZK proof in the arguments of a transaction submitted to $SC$. 
%
\begin{figure}[h]
	\scriptsize
	\centering		
	%$$\boxed{u=1}$$
	\vspace{-1.1cm}
	\begin{equation}
	\boxed{
		\begin{array}{rcl}
		P_1: g^{x_1y_1}\cdot f_1= (g^{-x_1x_2-x_1\underline{x_3}-x_1x_4-x_1\underline{x_5}-x_1x_6})\cdot f_1\\
		P_2:\enspace\; g^{x_2y_2}\cdot f_2=  (g^{x_1x_2-x_2\underline{x_3}-x_2x_4-x_2\underline{x_5}-x_2x_6})\cdot f_2\\
		\triangleright P_3:\enspace\;
		g^{x_3y_3}\cdot f_3=  (g^{x_1x_3+x_2x_3-{x_3}x_4-x_3x_5-x_3x_6})\cdot f_3\\
		P_4: \enspace\;g^{x_4y_4}\cdot f_4=  (g^{x_1x_4+x_2x_4+\underline{x_3}x_4-x_4\underline{x_5}-x_4x_6})\cdot f_4\\
		\triangleright P_5:\enspace\;
		g^{x_5y_5}\cdot f_5=  (g^{x_1x_5+x_2x_5+x_3x_5+x_4{x_5}-x_5x_6})\cdot f_5\\
		P_6: \enspace\;g^{x_6y_6}\cdot f_6= (g^{x_1x_6+x_2x_6+\underline{x_3}x_6+x_4x_6+\underline{x_5}x_6})\cdot f_6\\			
		\end{array}
	}
	\end{equation}
	\vspace{-0.4cm}
	
	\caption{An example of faulty participants $P_3$ and $P_5$. Each honest participant inverts out all components of blinding keys containing underlined private keys of $P_3$ and $P_5$.}
	%		where $g^{x_1y_1}$ to $g^{x_6y_6}$ are the blinding keys of participants $P_1$ to $P_6$.
	\label{fig:linear}
			\vspace{-0.5cm}
\end{figure}

The underlined variables in \autoref{fig:linear} show the distribution of ephemeral private keys from both $P_3$ and $P_5$, which are presented in the blinding keys of benign $P$s.
In detail, $SC$ verifies whether the supplied $g^{x_ix_j}$ corresponds to $P_i$'s and $P_j$'s public keys ($g^{x_i}$ and $g^{x_j}$) using the ZKP verification from \autoref{fig:ZKPdiffie}.
Once this phase is completed without new faulty $P$s, the phase of our protocol is shifted to the tally phase, and it continues as before, but without the votes of faulty $P$s.





%Unlike other protocols that require participation from all remaining participants in key recovery such as Khader et al.~\cite{KhaderSRH12} in the reconstruction phase, we employ a publicly verifiable secret sharing scheme (PVSS) where any threshold number of participants are able to recover the secret. 
%\zli{Schoenmakers~\cite{C:Schoenmakers99}, PVSS seems not right, ....}
%\sarad{removed duplicate citation.}
%In PVSS, involved parties may verify consistency of the encrypted shares (in the deal phase) as well as the consistency of decrypted shares (in the reconstruction phase).
%This allows us to penalize all faulty participants.
%Such a scheme is presented in Schoenmakers~\cite{Schoenmakers99}.
%If one of $P_i$ or $P_j$ passes the verification, $g^{x_ix_j}$ can be recovered.
%Necessary verification is interfaced by writing to the $SC$ and retrieving it, while the other operations may be carried out offline.





==> sec/governance.tex <==


In this section, we discuss the salient features supported by liquid democracy and compare it with corrective governance to bring out their similarities and differences.

\subsubsection*{Liquid Democracy}
In liquid democracy, a participant may either vote directly or delegate their vote to an expert.
Participants may at any time revoke their delegation and vote directly or choose a new delegate.
Any expert may inturn re-delegate the votes to another expert of their choice.
The expert maintains accountability by revealing their decisions and votes to the participants, hence their votes are not a secret~\cite{Ford2002}.
%The goal of the expert is to optimize the accuracy in representation of votes delegated to them with respect to the effort spent in making the correct voting decision. % IH: this is unclear; the goal of expert is to vote; also there is no correct voting decision, so it does not make sense to me.
A participant may delegate their vote based on their time, effort and interest in the item put up for voting.
We refer the reader to a study Bloembergen et al.~\cite{BloembergenGL19} that discusses rationality of delegation.
Expert opinion may at times be conflicting~\cite{Matheson2005,Goldman2001} and the participants are required to make an effort to arrive at an informed decision.
However, they are able to revoke their delegation when they want.
%\IH{So far you were talking about liquid democracy, so now I would expect the new paragrah about corrective governance + possible comparison.}
\subsubsection*{Corrective Governance}
In corrective governance, the time between two main elections is split into a continuous and repeating set of time epochs. 
Any participant is able to change her vote in any future time epoch.
This results in a new winner when a supermajority percentage of votes was cast in a representative's favor, when voting in time epochs between two main elections. 
For the main election time epoch, it only needs a majority to announce the winning representative.


\subsubsection*{Comparison}
Liquid democracy has a lower barrier to participation since it supports vote delegation.
In contrast, corrective governance requires the participant to be available in a certain period of each epoch of continuous voting. 
%Our implementation using the blockchain incentivizes participants to vote continuously by rewarding their participation (see \autoref{ssec:benefits}). % IH: skip our stuff here; it should be only known theory hereorr
In liquid democracy, proposals have to table over to be considered again~\cite{ZhangOB19}.
However, there may be an unwillingness to retable proposals (put it up for voting again) where there is an opposition to it, since the final tally was already published.
In corrective governance, a voting is only tabled once, and it follows the rules of continuous voting.
As a result, voting on the proposal is always ongoing and avoids the barriers in having it retabled.	
%
Corrective governance  provides smoother transition and requires a supermajority to change a decision whereas in liquid democracy, changes in expert opinion may radically change the outcome~\cite{Golz2018,KlingKHSS15}.
Corrective governance requires regular deliberation to make informed choices (i.e., subjective opinion is formed based on important facts~\cite{Dryzek2000}) whereas liquid democracy supports the option to delegate their vote to an expert.
In liquid democracy, an expert may possibly wield substantial power and coerce participants in their sphere of influence to delegate their vote.
Corrective governance does not involve delegation and is resilient to such an issue.
Here, coercion attacks are thwarted by using the receipt-freeness or receipt-indistinguishability property (see \autoref{sec:rindistinguishability}).
We envision the corrective governance to be used in situations where it fits the purpose and complements the existing suite of governance systems.

%compliment and work in tandem for improved governance
%Applications DAO


%\renewcommand{\arraystretch}{0.5}
%\setlength{\tabcolsep}{0.2cm}




==> sec/implementation.tex <==


%http://eth-converter.com/
We selected the Ethereum-based environment for evaluation due to its wide\-spread adoption and open standardized architecture (driven by the Enterprise Ethereum Alliance~\cite{EEA}), which is incorporated by many blockchain projects.
We implemented $SC$ components in Solidity, while $VA$ and $P$ components were implemented in Javascript as testing clients of the \textit{truffle} project.
%\footnote{The source code of our implementation is available at \url{https://www.dropbox.com/sh/f2gmjnhov70ndjk/AAAqe6bdMKQFgAJ9dBqvTOHda?dl=0}.}
%
% and contains XXX lines of code. % (see \autoref{tab:loc} in Appendix).
%\sarad{adding file can be later but will leave a note not to forget }\ih{ok}
Executing smart contracts over blockchain, i.e., performing computations and storing data, has its costs. 
In Ethereum Virtual Machine (EVM), these costs are expressed by the level of execution complexity of particular instructions, referred to as \textit{gas}.
%\footnote{One unit of gas has its market price in GWEI, while one unit of GWEI has its market price in fiat currency.}
%	
In this section, we analyze the costs imposed by our approach, perform a few optimizations, and compare the costs with OVN~\cite{McCorrySH17}.
%To the best of our knowledge there are no other implementations from the same class of protocols, for voting choices $>$ 2.
%
%\sarad{Ivan, we somehow need to compare costs with this paper Seifelnasr et al.~\cite{DBLP:conf/fc/SeifelnasrGY20}? it seems lower than  ours due to merkle tree root and off-chaining...but we still have to compare and justify ours? maybe one paragraph? i have a couple of sentences on it in related work.
%https://eprint.iacr.org/2020/033.pdf
%Sarad:since their setting is different, we probably dont need to compare
%}
In the context of this work, we assume 10M as the block gas limit.
With block gas limit assumed for a single transaction, our implementation supports up to 135 participants (see \autoref{fig:mpc-comparison}), up to 7 vote choices (see \autoref{fig:submit-vote}), and up to 9 simultaneously stalling faulty participants (see \autoref{fig:repair-vote}).\footnote{This maximum corresponds to a single recovery round but the total number of faulty participants can be unlimited since the fault recovery round can be repeated.}
%For our cost optimizations, refer \autoref{ssec:optimizatations}.
%
%In sum, we made two implementations, one basing on integer arithmetic (IA) in $\mathbb{F}_p^*$ (see \autoref{ssec:basicprotocol}) and another one basing on elliptic curve cryptography (ECC) in $\mathbb{F}_p^*$ (see Appendix~\ref{sec:appendixecc}), where we utilized standardized \textit{Secp256k1} curve.
%Since discrete logarithm was already computed for 768-bit long modulus in 2016~\cite{kleinjung2017computation}, we assumed 1024 bits as the minimal secure bit length for integer arithmetic implementation.




%\myparagraph{\textbf{IA vs. ECC Implementation}} \ih{move?}
%We observed that the minimal secure length of big numbers in IA implementation (i.e., 1024 bits) causes a high overhead required by the big numbers library~\cite{bignumber-solidity}, which is reflected in high costs.
%This led us to the conclusion that IA implementation is overly expensive,  and thus in many cases does not fit the block gas limit. % of Ethereum.
%Therefore, we assume ECC implementation more efficient and preferred solution.

We made two different implementations, the first one  is based on DLP for integers modulo $p$ (denoted as integer arithmetic (IA)), and the second one is based on the elliptic curve DLP (denoted as ECC).
We refer the reader to \autoref{sec:appendixecc} for the ECC notation of our work, which is analogous to IA notation from \autoref{sec:protocol}. 
In the ECC, we used a standardized \textit{Secp256k1} curve from existing libraries~\cite{witnet-ecc-solidity}, \cite{McCorrySH17}.
In the case of IA, we used a dedicated library~\cite{bignumber-solidity} for operations with big numbers since EVM natively supports only 256-bit long words, which does not provide sufficient security level with respect to the DLP for integers modulo $p$.\footnote{Since this DLP was already computed for 795-bit long safe prime in 2019~\cite{integer-dlp-2019}, only values higher than 795-bit are considered secure enough.}
We consider 1024 bits the minimal secure (library-supported) length of numbers in IA.
%
As we will show below, IA implementation even with minimal 1024 bits is overly expensive, and thus in many cases does not fit the block gas limit by a single transaction. 
Therefore, in our experiments, we put emphasis on ECC implementation that is more efficient and preferred option.
%
The source code of our implementation is available at \url{https://www.dropbox.com/sh/f2gmjnhov70ndjk/AAAqe6bdMKQFgAJ9dBqvTOHda?dl=0}.


% (see comparison with ECC in \autoref{fig:mpc-comparison} and \autoref{fig:submit-vote}).  
%, in the case of which, all required modular arithmetic operations can be performed natively in Ethereum (after the Byzantium hard fork in 2017).


 
 
%To address the last bottleneck (i.e., vote submission), we introduce batching parametrized by $w$, the number of 1-of-k ZKP (i.e., equal to the number of candidates) that are to be verified in a single transaction.
%\IH{todo}
%Thanks to this scalability improvement, we can support up to $X$ candidates (when $w = 1$).
%%
%The experiment measuring the cost of batched submission of a vote is depicted in \autoref{fig:}, where we can observe that...



	
%\subsection{Cost Analysis}
%Deployment cost of a single voting booth contract and aggregation contract are $4.36M$ and $YY$ units of gas, respectively; both fitting the block limit (i.e., $6.7M$ of gas).
%Next, submission of the ephemeral key costs $118K$ of gas, while all remaining operation have variable costs, which we investigate in the following.


%\IH{this is the old one for IA}
%
%\noindent\textbf{Compute MPC Keys:} This operation is performed by $VA$ when voting $SC$ turns into the pre-voting stage. 
%The cost of this operation is dependent on the number of participants that submitted their ephemeral public keys (and thus are eligible to vote).
%\autoref{fig:cost-MPC} shows the cost of compute MPC key transaction parametrized by a range of participants and size of public modulus $p$.
%We see that for 256 bits, the maximum number of participants that can be part of a single booth (i.e., fitting the block limit) is 55.
%%


%\noindent\textbf{Vote submission:} This operation is performed by each eligible voter during the voting stage.
%The cost of vote submission depends on the number of candidates since proof verification is executed per each candidate (see \autoref{fig:ZKPMultiCandidate}).
%%
%In \autoref{fig:cost-submit-vote}, we depict the cost of vote submission parametrized by various number od candidates, while using three different values for size of public modulus $P$.
%Note that results are averaged per participants.
%With 256 bit modulus, our implementation allows for the maximum of $22$ candidates\sarad{per booth?}.
%
%%
%\begin{figure}[th]
%	\begin{center}		
%		\includegraphics[width=0.47\textwidth]{fig/gasVoteSubmission.pdf} 
%		\caption{Cost of vote submission.}
%		\label{fig:cost-submit-vote}
%		%		\vspace{-0.2cm}
%	\end{center}	
%\end{figure}



\subsection{Cost Optimizations}
\label{ssec:optimizatations}	
\input{sec/optimizations}




Since ECC operations in ZKP verifications (see \autoref{fig:ECCZKPMultiCandidate} and \autoref{fig:ZKPECC} of \autoref{sec:appendixecc}) and computation  of MPC keys (see \autoref{eqn:eccmpc} of \autoref{sec:appendixecc}) impose a high execution cost in the setting of decentralized blockchains, we have made several cost optimizations.



\subsubsection{\textbf{(1) Caching in MPC Key Computation.}}
If implemented nai\-vely, the computation of all MPC keys in $SC$ (see \autoref{eqn:eccmpc} of \autoref{sec:appendixecc}) would contain a high number of overlapped additions, 
\begin{wrapfigure}{t}{0.65\textwidth}
	\centering
	%	\vspace*{-0.1cm}
	\includegraphics[width=\linewidth]{fig/gas/mpc-comparison.pdf}
	%	\vspace{-0.3cm}
	\caption{A computation of MPC keys by the authority.} % across various implementations and optimizations.}
	\label{fig:mpc-comparison}
	\vspace*{-0.4cm}
\end{wrapfigure}
and hence the price would be excessively high (see series \textit{``ECC-Affine (naive)''} in \autoref{fig:mpc-comparison}).\footnote{The same phenomenon occurs in IA (see \autoref{eqn:eq1}) but with overlapped multiplications (see series \textit{``IA 1024 bits (naive)''}).}
Therefore, in the code of $SC$ related to the computation of all MPC keys, we accumulate and reuse the value of the left side of \autoref{eqn:eccmpc} during iteration through all participants. 
Similarly, the sum at the right side can be computed when processing the first participant, and then in each follow-up iteration, it can be subtracted by one item. 
%
%
However, we found out that subtraction imposes non-negligible costs since it contains one affine transformation (which we later optimize). 
In the result, we found pre-computation of all intermediary right items in the expression during the processing of the first participant as the most optimal. %\ih{pseudocode?}
%
The resulting savings are depicted as \textit{``ECC-Affine (caching)''} series in \autoref{fig:mpc-comparison}.
We applied the same optimization for IA; however, even after adding a further optimization (i.e., pre-computation of modular inverses; see \autoref{ssec:optimizatations}.4), the costs were still prohibitively high (see \textit{``IA 1024 bits (caching+modi)''} series in \autoref{fig:mpc-comparison}) and the maximum number of participants fitting the block gas limit was equal only to 29.



%\begin{figure}[t]
%	\centering
%	\vspace{-0.3cm}
%	\includegraphics[width=0.62\columnwidth]{fig/gas/mpc-comparison.pdf}
%	%	\vspace{-0.3cm}
%	\caption{A computation of MPC keys by the authority.} % across various implementations and optimizations.}
%	\label{fig:mpc-comparison}
%	\vspace{-0.7cm}
%\end{figure}

\begin{figure}[b]
		\vspace{-1.2cm}
	\centering	
	%	\hspace{-0.9cm}
	\subfloat[Vote submission by $P_i$.\label{fig:submit-vote}]{	
		\includegraphics[width=0.48\columnwidth]{fig/gas/submit-vote.pdf}
		\vspace{0.3cm}
	}
	%	\hspace{1.3cm}
	\subfloat[Vote repair by $P_i$.\label{fig:repair-vote}]{	
		\includegraphics[width=0.48\columnwidth]{fig/gas/repair-vote.pdf}	
		\vspace{0.3cm}
	}		
	%	\vspace{-0.2cm}
	\caption{Vote submission and vote repair (i.e., fault recovery) with various optimizations.}
	\label{fig:submit-and-repair-vote}
			\vspace{-0.6cm}
	
\end{figure}

\subsubsection{\textbf{(2) Affine vs. Jacobi Coordinates.}}
In the ECC libraries employed~\cite{witnet-ecc-solidity} \cite{McCorrySH17}, by default, all operations are performed with points in Jacobi coordinates and then explicitly transformed to affine coordinates.
However, such a transformation involves one modular inversion and four modular multiplications over 256-bit long integers, which is costly.
Therefore, we maximized the utilization of internal functions from the Witnet library~\cite{witnet-ecc-solidity}, which do not perform affine transformation after operation execution but keep the result in Jacobi coordinates.
This is possible only until the moment when two points are compared since a comparison of points in Jacobi coordinates can be made only after the points are transformed to affine coordinates. 
Hence, a few calls of the affine transformation are inevitable -- e.g., in the case of ZKP verification during the vote submission (see the $SC$ side in \autoref{fig:ECCZKPMultiCandidate} of \autoref{sec:appendixecc}), there is one affine transformation required in the first check and two affine transformations in the second check.
%
This optimization is depicted in \autoref{fig:mpc-comparison} (series \textit{``ECC-Jacobi (caching)''}) and \autoref{fig:submit-vote} (series \textit{``ECC-Jacobi''}). % where series are distinguished with different coordinate systems.
In the case of computation  of MPC keys, this optimization brought improvement of costs by $23\%$ in contrast to the version with affine coordinates and caching enabled.
Due to this optimization, up to $111$ participants can be processed in a single transaction not exceeding the block gas limit.
%\footnote{As we will see in \autoref{sec:scalability-improvements} the more participants are processed in a single transaction, the lower the costs.}.
%
In the case of vote submission, this optimization brought improvement of costs by $33\%$ in contrast to the version with affine coordinates.


\subsubsection{\textbf{(3) Multiplication with Scalar Decomposition.}}
The most expensive operation on an elliptic curve is a scalar multiplication; based on our experiments, it is often 5x-10x more expensive than the point addition (in terms of gas consumption) since multiplication itself involves several point additions (and/or point doubling).
The literature proposes several ways of optimizing the scalar multiplication, where one of the most significant ways is w-NAF (Non-Adjacent Form) scalar decomposition followed by two simultaneous multiplications with scalars of halved sizes~\cite{hankerson2005guide}.
This approach was also adopted in the Witnet library~\cite{witnet-ecc-solidity} that we base on.
The library boosts the performance (and decreases costs) by computing the sum of two simultaneous multiplications $kP + lQ$, where $k = (k_1 + k_2 \lambda)$, $l = (l_1 + l_2 \lambda)$, and $\lambda$ is a specific constant to the endomorphism of the elliptic curve.
To use this approach, a scalar decomposition of $k$ and $l$ needs to be computed beforehand.
%
Nevertheless, such a scalar decomposition can be computed off-chain (and verified on-chain), while only a simultaneous multiplication is computed on-chain.
However, to leverage the full potential of the doubled simultaneous multiplication, one must have the expression $kP + lQ$, which is often not the case.
%
In our case, such a form fits the second check of vote's ZKP verification at $SC$ (see the right side of \autoref{fig:ECCZKPMultiCandidate} in \autoref{sec:appendixecc}) since the expression of the second check can be rewritten to
$
r_1 H + d_i F_l \stackrel{?}{=} B_l + d_l V_i,
$
which enables us to apply a simultaneous multiplication on the left side.
The first check of the expression in \autoref{fig:ECCZKPMultiCandidate} can be also modified to leverage simultaneous multiplication as follows:
$
r_l G - d_l X  \stackrel{?}{=} A_l.
$
However, in this case, we have to invert both decomposed scalars of $d_l$ to satisfy $d_l = d_l^1 + d_l^2 ~\lambda ~mod~ n$.
Alike the vote submission, this optimization can be applied in vote repair (see \autoref{fig:ZKPECC}), where both checks can be rewritten to their equivalent form containing sums of multiplications: $rG -hA \stackrel{?}{=} m_1$ and $rB -cC  \stackrel{?}{=} m_2$.
%
We depict the performance improvement brought by this optimization as series \textit{``ECC-Jacobi (smul)''} in \autoref{fig:submit-and-repair-vote}.
%

%Another aspect that we had to deal with in the vote submission is the fact that all $d$ parameters are part of the checksum that is verified at $SC$ (see \autoref{fig:ECCZKPMultiCandidate} of \autoref{sec:appendixecc}). 
%Therefore, $SC$ first executes a multiplication of decomposed scalars to obtain full $d$ parameters and then use them to validate the checksum \ih{drop?}.



\subsubsection{\textbf{(4) Pre-Computation of Modular Inversions.}}\label{sec:optim-modular-inv}
Each affine transformation in the vote submission contains one operation of modular inversion -- assuming previous optimizations, ZKP verification of one item in 1-out-of-$k$ ZKP (see \autoref{fig:ECCZKPMultiCandidate} of \autoref{sec:appendixecc}) requires three affine transformations (e.g., for $k=5$, it is $15$). 
Similarly, the ZKP verification of correctness in the repair vote (see \autoref{fig:ZKPECC} of \autoref{sec:appendixecc}) requires two affine transformations per each faulty participant submitted.
The modular inversion operation runs the extended Euclidean algorithm, which imposes non-negligible costs.
However, all modular inversions can be pre-computed off-chain, while only their verification can be made on-chain (i.e., modular multiplication), which imposes much lower costs.
We depict the impact of this optimization as \textit{``ECC-Jacobi (smul+modi)''} series in \autoref{fig:submit-and-repair-vote} and ``...modi...'' series in \autoref{fig:mpc-comparison}.
In the result, it has brought $5\%$ savings of costs in contrast to the version with the simultaneous multiplication.
%After applying all optimizations, our approach support maximally 7 choices and 135 participants fitting the block gas limit.
%\ih{Put max of FT here.}


%\sarad{Sarad. This upper bound for tally computation table (Tab.1) is extrapolated and has no value. more reasons for reviewers to attack paper. please remove table.} \ih{I explicitly marked estimated ones. I think it is important to give the reader a clue how long it might take - besides we are presenting moslty boardroom voting.}

\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{0.1cm}
\begin{table}[t]
	\centering	
	\scriptsize
	\vspace{-0.7cm}
	
	\subfloat[1 core]{	
		\begin{tabular}{r l l l l}		
			\toprule
			\textbf{Voters} & \multicolumn{4}{c}{\textbf{Choices}}  \\ [0.5ex]
			
			(n) & ~$k=2$ & ~$k=4$ & ~$k=6$ & ~$k=8$  \\ [0.5ex]
			\midrule
			\textbf{20} & $0.01s$ & $0.01s$ &  $0.07s$ & $0.07s$\\						
			\textbf{30} & $0.01s$ & $0.01s$ & $0.53s$ & $13.3s$\\								
			\textbf{40} & $0.01s$ & $0.04s$ & $02.6s$ & $112s$\\							
			\textbf{50} &$0.01s$ & $0.08s$ & $10.0s$ & $606s$\\
			
			\textbf{60} &$0.01s$ & $0.16s$ & $28.2s$ & $2424s$\\
			\textbf{70} &$0.01s$ & $0.48s$ & $69.6s$ & $\sim2.1h$\\
			\textbf{80} &$0.01s$ & $0.82s$ & $160s$ & $\sim5.8h$\\
			\textbf{90} &$0.01s$ & $1.08s$ & $320s$ & $\sim14.2h$\\
			
			
			
			\textbf{100}& $0.01s$ & $1.2s$ & $722s$ & $\sim33h$\\
			%\textbf{200}& $0.01s$ & $27s$ & $~12h$ (est.) & $~304d$ (est.)\\	
			
			%\textbf{1000}& $0.15s$ & $~4h$ (est.) & $>1Yr$ & $>1Yr$\\
			%2000& $0.57s$ & $-$ & $-$ & $-$\\
			%5000& $4.98s$ & $-$  & $-$ & $-$\\
			%[1ex]						
			\bottomrule
		\end{tabular}
	}
	\hspace{0.2cm}
	\subfloat[8 cores]{
		
		\begin{tabular}{r l l}		
			\toprule
			\textbf{Voters} & \multicolumn{2}{c}{\textbf{Choices}}  \\ [0.5ex]
			
			(n)  & ~$k=6$ & ~$k=8$  \\ [0.5ex]
			\midrule
			\textbf{20}  &  $0.01s$ & $0.01s$\\						
			\textbf{30}  & $0.08s$ & $2.0s$\\								
			\textbf{40} & $0.39s$ & $16.8s$\\							
			\textbf{50}  & $1.5s$ & $90.9s$\\					
			\textbf{60}  & $4.44s$ & $267s$\\					
			\textbf{70}  & $11.85s$ & $773s$\\								
			\textbf{80}  & $19.46s$ & $2210s$\\								
			\textbf{90}  & $44.02s$ & $\sim2.7h$\\								
			\textbf{100} &  $108.3s$ & $\sim4.9h$\\			
			%\textbf{200}& $0.01s$ & $27s$ & $~12h$ (est.) & $~304d$ (est.)\\				
%			\textbf{1000}& $0.15s$ & $\sim4h$ & $>1Yr$ & $>1Yr$\\
			%2000& $0.57s$ & $-$ & $-$ & $-$\\
			%5000& $4.98s$ & $-$  & $-$ & $-$\\
			%[1ex]						
			\bottomrule
		\end{tabular}
	}
	\caption{Upper time bound for tally computation.}	\label{table:bruteforcetime}
	\vspace{-0.9cm}
	
\end{table}



\subsection{Tally Computation}\label{sec:tally-exps}
\vspace{-0.3cm}
In \autoref{table:bruteforcetime}, we provide time measurements of tally computation through the entire search space on a single core vs. all cores of the Intel Core i7-10510U CPU laptop.\footnote{Note that in some cases we estimated the time since we knew the number of attempts.} % 1.8 GHZ (base frequency)
We see that for $n \le 100$ and $k \le 6$, the tally can be computed even on a commodity PC in a reasonable time.
However, for higher $n$ and $k$, we recommend using a more powerful machine or distributed computation across all $P$s. % and thus achieve faster response.
One should realize that our measurements correspond to the upper bound, and if some ranges of tally frequencies are more likely than other ones, they can be processed first -- in this way, the computation time can be significantly reduced.
Moreover, we emphasize that an exhaustive search for tally computation is not specific only to our scheme but to homomorphic-encryption-based schemes providing perfect ballot secrecy and privacy of votes (e.g.,~\cite{Kiayias2002},~\cite{HaoRZ10},~\cite{McCorrySH17}).
%We also note, that if the practical use case would require shorter time to obtain the tally results, the time complexity can be further reduced by baby-step giant-step method (proposed by Shanks) to $\mathcal{O}(\sqrt{n}^{k-1})$ attempts, which might be of interest especially when scaling the number of participants in our scheme.
%However, for the proof-of-concept purposes, we implemented and evaluated only a naive exhaustive search and its parallelized version.


\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{0.15cm}
\begin{table}[b]
	\vspace{-0.6cm}
	\centering
	\scriptsize
	
	\begin{tabular}  {l c l l}
		\toprule
		& \textbf{Gas Paid by} & \textbf{OVN} &\textbf{\name}   \\
		\midrule
		
		%		Max. Participants   &  124 &  135\\
		%		Max. Choices  &  2 &  7 \\
		\textbf{\specialcell{Deployment of Voting $SC$}}   	& $VA$ &  3.78M  & 4.8M  \\
		
		\textbf{\specialcell{Deployment of\\Cryptographic $SCs$}}  & $VA$ &  \specialcell{2.44M}  & \specialcell{2.15M\\(1.22M+0.93M)}   \\
		
		\textbf{Enroll voters} & $VA$ & \specialcell{2.38M\\(2.15M+0.23M)}  & 1.93M \\
		
		\textbf{\specialcell{Submit Ephemeral PK}} & $P$ &  0.76M & 0.15M  \\
		
		\textbf{Cast Vote} & $P$ &  2.50M & 2.72M \\
		
		\textbf{Tally} & $VA ~(or ~P)$ & 0.75M  & 0.39M  \\				
		
		\midrule
		\textbf{Total Costs for} $\mathbf{P}$ &   & 3.26M  & 2.87M \\
		
		\textbf{Total Costs for} $\mathbf{VA}$ &  &  9.35M  & 9.27M  \\
		
		%		Nobody is interested in abstract values below, since current gas price is crazy. We should stay in gas units.
		%		Norm. voter costs   &  \$29.72$\cdot$ (175/11)$\cdot$ (1/5)=\$94.56 &  \$76\\
		%		Norm.  cost to $VA$    &  \$2.74$\cdot$ (175/11)$\cdot$ (1/5)=\$8.71 &  \$3.16\\
		%		Total Norm. costs    &  \$94.56+\$8.71=\$103.27 &   \$76+\$3.16=\$79.16\\
		
		\bottomrule
		\vspace{-0.2cm}
	\end{tabular}
	\caption{A normalized cost comparison of \name with OVN for $n=40$ and $k=2$.}\label{tab:costcomparisons}
	\vspace{-0.8cm}
\end{table}



\subsection{Cost Comparison}
\vspace{-0.3cm}
In \autoref{tab:costcomparisons}, we made a cost comparison of \name (using ECC) with OVN~\cite{McCorrySH17}, where we assumed two choices and 40 participants (the same setting as in~\cite{McCorrySH17}).
We see that the total costs are similar but \name improves $P$'s costs by $13.5\%$ and $VA$'s cost by $0.9\%$ even though using more complex setting that allows 1-out-of-k voting.
%
We also emphasize that the protocol used for vote casting in \name \textbf{contains more operations} than OVN but regardless of it, the costs are close to those of OVN, which is mostly caused by the proposed optimizations.\footnote{To verify 1-out-of-$k$ ZKP in vote casting, \name computes $5 \cdot k$ multiplications and $3 \cdot k$ additions on the elliptic curve -- i.e., 10 multiplications and 6 additions for  $k=2$. In contrast, OVN computes only 8 multiplications and 5 additions for $k=2$.}
%
Next, we found that OVN computes tally on-chain, which is an expensive option.
In contrast, \name computes tally off-chain and $SC$ performs only verification of its correctness, which enables us to minimize the cost of this operation.
Another gas saving optimization of \name in contrast to OVN (and Hao et al.~\cite{HaoRZ10}) is that we do not require voters to submit ZKP of knowledge of $x_i$ in $g^{x_i}$ during the registration phase to $SC$ since $P_i$ may only lose by providing incorrect ephemeral public key $g^{x_i}$ -- she might lose the chance to vote and her deposit.
%
Finally, we note that we consider the deployment costs of our $SC$ equal to 4.8M units of gas; however, our $SC$ implementation contains a few auxiliary view-only functions for a pre-computation of modular inverses, with which, the deployment costs would increase to 7.67M due to code size.
Nevertheless, these operations can be safely off-chained and we utilized them on-chain only for simplicity. % thereby removed from $SC$ in a production deployment, and we kept them at $SC$ only for proof-of-concept purposes. 
%Then, we assume the average exchange rate of ETH/USD equal to $175$ and the ``standard'' gas price $4$ GWEI\footnote{\url{https://ethgasstation.info/}.} as of November 20, 2019.
%We can see that the number of candidates is the parameter influences the cost of the elections mostly.







%\setlength{\tabcolsep}{1.8pt}
%\begin{table}
%	\centering
%	\caption{Our Solution: Expenses paid by each participant.}
%	\begin{tabular}{@{}cccccccccc@{}}
%		\toprule
%		\textbf{Candidates}     & 2    & 3    & 4    & 5 
%		    & 6    & 7    & 8    & 9    & 10   
%		\\ \midrule
%		\textbf{Cost {[}USD{]}} & 1.90 & 2.83 & 3.77 & 4.70 
%		 & 5.60  & 6.54 & 7.45 & 8.39 & 9.28 
%		\\ \bottomrule
%	\end{tabular}
%	%\vspace{3pt}
%	\label{tab:overall-costs-voter}
%\end{table}
%\setlength{\tabcolsep}{2.4pt}

% cost of deploy for one booth $SC$ using contract factory $SC$ is 3919596.
%


%\setlength{\tabcolsep}{4pt}
%%\renewcommand{\arraystretch}{1.2}
%\begin{table}[t]
%	%	\vspace{-0.5cm}
%	\footnotesize
%	\centering{
%		\begin{tabular}{>{\raggedleft} r c c c @{}}
%			
%			\toprule
%			\textbf{Operation}                                                                                    & \textbf{\specialcell{Mean\\$[gas]$}} & \textbf{\specialcell{Standard\\Deviation\\~~~$[gas]$}}                \\ 
%			\Xhline{2\arrayrulewidth} \noalign{\smallskip}
%			
%			
%			\textbf{Deployment of $SC$}                 & 4,362,541        &  -                     \\ 
%			\textbf{Computation of Tally}                 & 4,362,541        &  -                     \\ 
%			\bottomrule
%		\end{tabular}
%	}
%	
%	\caption{Costs of all operations with smart contracts.}	
%	\label{tab:other-costs}
%	
%\end{table}


==> sec/introduction.tex <==
Voting is an integral part of democratic governance, where eligible participants can cast a vote for their representative choice (e.g., candidate or policy) through a secret ballot.
The outcome of voting announces a tally of votes.
%which is governed by the rules of the voting system.
Voting is usually centralized and suffers from a single point of failure that can be manifested in censorship, tampering, and issues with availability of a service.
% tamapering in voting machines, supported in	 https://followmyvote.com/voting-system-vulnerabilities/

%E-voting schemes are traditionally built for large-scale elections, with varying degrees of centralization. 
%Lesser research has been carried out for improving security in small-scale decentralized elections (up to  100 voters). 


Blockchain is an emerging decentralized technology that provides interesting properties such as decentralization, censorship-resistance, immutability of data, correct execution of code, and extremely high availability, which can be harnessed in addressing the existing issues of e-voting.
%
%We leverage existing work in boardroom voting to provide maximum vote privacy by employing a self-tallying voting protocol.
%
%
%We utilize an existing public blockchain that runs a decentralized consensus protocol, relying on an honest majority of all consensus nodes to achieve this goal. %~\cite{wood2014}.
%
A few blockchain-based e-voting solutions have been proposed in recent years, mostly focusing on boardroom voting~\cite{McCorrySH17,EPRINT:PanRoy18,Li2020,yu2018platform} or small-scale voting~\cite{DBLP:conf/fc/SeifelnasrGY20,icissp:DMMM18,Li2020}. 
%\ih{check whether \cite{DBLP:conf/fc/SeifelnasrGY20} is only for small scale.}




Decentralization was a desired property of e-voting even before invention of blockchains.
For example, (partially) decentralized e-voting that uses the homomorphic properties of El-Gamal encryption was introduced by Cramer et al.~\cite{cgs97}. % and many of its variants are in use \ih{citations? Helios?}.
It assumes a threshold number of honest election authorities to provide the privacy of vote.
However, when this threshold is adversarial, it does not protect from computing partial tallies, making statistical inferences about it, or even worse  -- the vote choices of participants.
A solution that removed trust in tallying authorities was for the first time proposed by Kiayias and Yung~\cite{Kiayias2002} in their privacy-preserving self-tallying boardroom voting protocol.
A similar protocol was later proposed by Hao et al.~\cite{HaoRZ10}, which was later extended to a blockchain environment by McCorry et al.~\cite{McCorrySH17} in their Open Voting Network (OVN).
%
%OVN preserves the privacy of cast votes.
An interesting property of OVN is that it requires only a single honest voting participant to maintain the privacy of the votes.
%Furthermore, it does not require the authority to tally the votes; instead, any participant can compute the tally when voting finishes (i.e., self-tallying). \ih{this is incorrect; the tally is computed by SC.}
%Our work is motivated by OVN's privacy-preserving property of the self-tallying votes and limiting the authority's role to setting up and triggering the phases of the election.
%
%OVN is implemented with the use of the Ethereum smart contract, it provides voter privacy and allows for two-vote choices.
However, OVN  supports only two vote choices (based on~\cite{HaoRZ10}), assumes no stalling participants, and requires expensive on-chain tally computation (limiting its scalability).
The scalability of OVN was improved by Seifelnasr et al.~\cite{DBLP:conf/fc/SeifelnasrGY20}, but retaining the limitation of 2 choices and missing robustness.

Our goal is to build a remote boardroom voting protocol that resolves these limitations and would enable a straightforward extension to support scalability.
Therefore, we introduce BBB-Voting, a blockchain-based boardroom voting system providing  1-out-of-$k$ voting, while additionally offering a mechanism for resolution of faulty participants.
%As the name suggests, it is unsuitable for elections that allow participants to vote for more than one candidate is the preferred rank order. \ih{intuitive}
%
Alike OVN, BBB-Voting also provides the maximum privacy of votes in the setting that outputs the full tally of votes (as opposed to \textit{tally-hiding} protocols~\cite{kusters2020ordinos,huber2022kryvos}). % and it requires a Turing-complete smart contract blockchain platform (further blockchain) to operate.
% is secure and verifiable.
Both OVN and BBB-Voting require the authority
%\footnote{W.l.o.g, it may be replaced by a quorum that requires a multi-sig threshold number of participants in agreement to invoke an action.} 
whose role is limited to registering participants into voting and shifting the phases of the protocol (also possible by the participants).
%All public key material and proofs are posted on a public blockchain.
The communication between the participants and the blockchain is semi-synchronous; i.e.,
each participant is expected to execute certain actions within a given time frame. % while the order of their participation is irrelevant.
When all registered participants submit their votes, the result can be tallied by anybody and the correctness of the result is verified by the blockchain.
%Hence, no manual decryption~\cite{KhaderSRH12} or unblinding of individual votes is required.
%Since OVN is the closest work and there is no other work (to the best of our knowledge) in a comparable setting, we compare our work with OVN. \ih{this is redundant}
%

% From scalable OVN paper:
%Traditionally, e-voting protocols rely on a trusted authority for collecting
%the encrypted votes from the voters to maintain the voters’ privacy. Later, that
%trusted authority computes the final tally from the casted votes. The problem in
%this approach is giving a single centralized authority the full control of collecting
%and computing the tally. Instead, multiple authorities can be utilized for collecting the votes and in the tally computation phase, e.g., see Helios [3]. Yet, the
%collusion of the tally authorities is still a threat against voters’ privacy. Removing
%the tally authorities completely was first accomplished by Kiayias and Yung [11]


\myparagraph{\textbf{Contributions}}
We make the following contributions.
%
\begin{compactenum}[i)]
	\item We present \name, an approach for remote end-to-end verifiable priva\-cy-preserving self-tallying 1-out-of-$k$ boardroom voting on the blockchain (see \autoref{sec:protocol}).	
	%
	In detail, we start with the voting protocol proposed by Hao et al.~\cite{HaoRZ10} that provides a low bandwidth requirements and computational costs but is limited to 2 vote choices.
	We extend this protocol to support $k$ choices utilizing the 1-out-of-$k$ proof verification proposed by Kiayias and Yung~\cite{Kiayias2002}. % as the extension of their 1-out-of-2 voting protocol. 
	We accommodate this approach to run on the blockchain with Turing-complete smart contract capability, enabling on-chain zero-knowledge proof verification of blinded votes (and other proofs).
%	Hao: with low bandwidth requirements and computational costs
	
	
	\item We incorporate a robustness approach~\cite{KhaderSRH12} into our protocol, which enables us to eliminate (even reoccurring) stalling (i.e., faulty) participants and thus finish voting without restarting the protocol (see \autoref{sec:faulttolerance}).
	
	\item We make two implementations, one based on discrete logarithm problem (DLP) for integers modulo $p$ and the second one based on the elliptic curve DLP.
	For both implementations we propose various optimizations reducing the costs imposed by the blockchain platform (\autoref{ssec:optimizatations}).
	Due to the optimizations, our implementation (with elliptic curve DLP) increases the number of participants fitting a single block by $9\%$ in contrast to OVN~\cite{McCorrySH17} under the same assumptions, while it decreases the costs for voters by $13.5\%$.

	\item We outline a scalability extension of our work, enabling the number of participants to be limited only by the expenses paid by the authority to register participants and compute their MPC keys as well as the computing power to obtain the tally.
	%
	For demonstration purposes, we evaluate its utility in the context of the voting that is a magnitude greater than the boardroom voting (i.e., up to 1000 participants) while preserving almost the same per-participant costs paid by the authority as without this extension (see \autoref{ssec:scalability-improvements}).  % and thus achieve better privacy properties than in the boardroom voting.

	
		
%	\item \ih{drop} We provide an extensive discussion about blockchain voting vs. centralized voting, and we address multiple concerns raised by the experts in the voting field (see \autoref{sec:centralized-vs-blockchain-voting}).
%	We demonstrate that using the blockchain as a public bulletin board does not influence the security of our protocol and can only improve the properties of e-voting in general.
	
%	\item We make a comparison of related work with \name in terms of various features specific to e-voting (see \autoref{sec:relatedwork}). % and we show that \name outperforms existing solutions in several aspects. 
\end{compactenum}









==> sec/model.tex <==
%\subsection{System Model}

\iffalse
\begin{figure}
	\centering
	\includegraphics[width=1\columnwidth]{fig/booth.pdf}
	\caption{Polling booths are replicated instances of a smart contract. Each contract instance corresponds to a single booth and serves a limited number of participants. New instances (booths) are added on demand to provide scalability.}
	\label{fig:booth}
\end{figure}
\fi


%\textit{\textbf{System model:}}
Our system model has the following actors and components:
%remember to add colored coins for different elections.
(1) \textit{a participant (P)}, who votes for a choice of her decision,
%Let $P_i$, denote the $i^{th}$ participant.
(2) \textit{a voting authority ($VA$)} who is responsible for validating the eligibility of $P$s to vote, their registration, and % them, and triggering voting phase changes in the protocol, and
%Due to the de-centralized nature of trust in blockchain, its role is limited to authenticating participants, i.e., verifying their eligibility to participate. \IH{This sentence says the same than the previous one.}
(3) \textit{a smart contract (SC)}, which collects the votes, acts as a verifier of zero-knowledge proofs, enforces the rules of voting, and verifies the tally.
%\autoref{fig:model} depicts the model of our proposed voting system.


%\subsection{Overview}
%\ih{drop?}
%We propose BBB-Voting, the approach for privacy-preserving end-to-end verifiable self-tallying boardroom voting on blockchain, supporting $ k \ge 2$ vote choices. 
%The protocols works as follows:
%(1) Eligible participants create a blockchain wallet and register their wallet addresses with $VA$.
%(2) $VA$ verifies the identity of each participant (i.e., \textit{know your client} (KYC)) and enrolls all voters to $SC$ by submitting their addresses.
%(3) Participants submit their ephemeral public keys that are further used to compute the multi-party computation (MPC) keys within SC.
%(4) Each participant submits her blinded vote and 1-out-of-$k$ zero-knowledge proof (ZKP) of set membership to SC, which verifies the correctness of the blinded vote.
%(5) If our protocol experiences faulty (i.e., stalling) participants during the voting, each participant repairs her blinded vote by submitting a counter-party key share\ih{??} of faulty participants to SC, including the ZKPs of correctness.
%$SC$ verifies ZKPs and accepts the repair of a blinded vote. % only in a successful case.
%(6) The authority $VA$ (or any voter $P_i$) submits the tally result to SC, which validates its correctness and informs other voters about the tally. % (i.e., the seventh step).
%
%%Double voting attempts are prevented natively since SC keeps track of all wallet addresses. % involved in the protocol.
%All faulty behaviors of participants are subject to deposit-based penalties (i.e., loss of deposits).
%In detail, a participant who submitted her ephemeral key and then has not voted within the timeout will lose the deposit, while the participants who voted will get their deposit back after voting finishes. 

%\subsubsection*{Fault Tolerance}
%TODO 

%\subsubsection*{Receipt-Indistinguishability}
%Optional features that our protocol supports are fault tolerance and receipt-indistinguishability.
%They are discussed in Appendix~\ref{sec:faulttolerance} and Appendix~\ref{sec:rindistinguishability}. 
%\IH{this is not enough about these features. I'd describe and define them here, and also write the difference with receipt free-ness that we do not provide.}


\subsection{Adversary Model}\label{sec:adversary-model}
The adversary $\mathcal{A}$ has bounded computing power, is unable to break used cryptographic primitives, and can control at most $t$ of $n$ participants during the protocol, where $t\leq n-2$ $\wedge$ $n\geq3$ (see \autoref{sec:appendixvoteorivacy}).
	%
%\sarad{Self note: Ask ZP to check this line.} 
%The adversary is centralized and can pool all the information from the participants under her control and use them in any manner. 
%The adversary is static.
%\sarad{from the security analysis, the adversary appears to be static, ZP, please check.} and is allowed to corrupt participants during an execution of the protocol. 
Any $P$ under the control of $\mathcal{A}$ can misbehave during the protocol execution. 
$\mathcal{A}$ is also a passive listener of all communication entering the blockchain network but cannot block it or replace it with a malicious message since all transactions sent to the blockchain are authenticated by signatures of $P$s or $VA$.
Finally, we assume that $VA$ \textbf{is only trusted in terms of identity management}, i.e., it performs identity verification of $P$s honestly, and neither censor any $P$ nor register any spoofed $P$.
Nevertheless, no trust in $VA$ is required to execute the rest of the protocol. %, alike in OVN~\cite{McCorrySH17}.
%


\iffalse
\subsection{Design Rationale}
\label{ssec:benefits}

\begin{figure}
	\centering
	\includegraphics[width=0.75\columnwidth]{fig/booth.pdf}
	\caption{Polling booths are replicated instances of a smart contract. Each contract instance corresponds to a single booth and serves a limited number of participants. New instances (booths) are added on demand to provide scalability.}
	\label{fig:booth}
\end{figure}
%Blockchain supports the following properties making it an attractive choice for the proposed electoral system:
One of our main design decision is to employ a blockchain platform.
The rationale for this decision is given below.


%\begin{compactitem}
	
	
	\noindent\textbf{A public bulletin board.}
	The use of a public bulletin board in voting was introduced by Cohen~\cite{Cohen1985} and Benaloh~\cite{Benaloh1986}.
	They are pivotal for public verifiability of voting, where the correctness of each step leading to the tally can be verified by anyone.
	As a consequence, voting remains dispute-free.
	In such a system, it is assumed that all participants can publish their messages to a designated area on the bulletin board but no one can alter its contents~\cite{Groth2004}.
	A blockchain serves as a reliable candidate to replace the bulletin board, as an append-only distributed ledger.
	Any (authorized) participant with an Internet connection can write to the blockchain. % while the  but not edit or remove information.
	
	\noindent\textbf{Identity management} is simplified by using a smart contract.
	This is an essential step to prevent unauthorized and duplicate voting by participants.
	Identities of participants map to their wallet addresses, which is verified by the authority.
	Next, the authority sends the verified wallet address to a designated voting smart contract.
	Subsequently, the smart contract
	%\sarad{does the smart contract or the blockchain do this signature verification?}
	verifies the possession of wallet private key by a particular participant whenever submitting a transaction (since tx is digitally signed).
	
\fi


==> sec/optimizations.tex <==




==> sec/preliminaries.tex <==

In this section, we describe terminology specific to voting. 
We assume that the reader is familiar with blockchains and smart contracts, and we refer an unfamiliar reader to \autoref{sec:appendix-blockchains} for a brief background.

\smallskip
%\subsection{Voting}
%\label{ssec:voting}
An \textit{involved party} refers to any stakeholder of the voting process and it covers \textit{all participants} and the \textit{authority}. % (see \autoref{sec:model}) 
%\label{ssec:requirements}
A voting protocol is expected to meet several properties.
A list of such properties appears in the works of Kiayias and Yung~\cite{Kiayias2002}, Groth~\cite{Groth2004}, and Cramer et al.~\cite{cgs97}. % and Park et al.~\cite{park2021going}:

%\begin{compactitem}
		\noindent\textbf{(1) Privacy of the Vote:} 
		ensures the secrecy of the ballot contents~\cite{Kiayias2002}.
		Hence, in a scheme that meets this property, a participant's vote must not be revealed other than by the participant herself upon her discretion (or through the collusion of all remaining participants).
		Usually, privacy is ensured by trusting authorities in traditional elections or by homomorphic encryption in some decentralized e-voting solutions (e.g.,~\cite{Kiayias2002,HaoRZ10,McCorrySH17,DBLP:conf/fc/SeifelnasrGY20,icissp:DMMM18}). 
		% voter-to-voter interactions or 
		%\ih{can we put some citations here?}
		%
%		\ih{drop?}Note that the privacy of votes might be violated even in the protocols using homomorphic encryption
%		% even though all ballots remain secret 
%		(i.e., in the case of unanimous voting by all participants).
%		This is an acceptable property \textit{iff} a voting protocol is required to output the final tally of votes (e.g., OVN~\cite{McCorrySH17} and BBB-Voting).
%		However, if a voting protocol is required to output only the winning choice or the order of choices, then the privacy holds only if the information about unanimous voting is not extractable from the output. % of a protocol. 				
		
		\noindent\textbf{(2) Perfect Ballot Secrecy:} is an extension of the privacy of the vote. 
		It implies that a partial tally (i.e., prior to the end of voting) is available only if all remaining participants are involved in its computation.	
				
		\noindent\textbf{(3) Fairness:} ensures that a tally may be calculated only after all participants have submitted their votes.
		Therefore, no partial tally can be revealed to anyone before the end of the voting protocol~\cite{Kiayias2002}.
		%This is achieved by ensuring that the tally can be computed only after a timeout.(not true)
		
		\noindent\textbf{(4a) Universal Verifiability:} any involved party can verify that all cast votes are correct and they are correctly included in the final tally~\cite{Kiayias2002}.
%		This is achieved by using a tamper-evident public bulletin board and zero-knowledge proofs to verify the validity of submitted votes.
		
		\noindent\textbf{(4b) End-to-End (E2E) Verifiability:}
		The verifiability of voting systems is also assessed by E2E verifiability~\cite{benaloh2015end}, which involves \textit{cast-as-intended}, \textit{recorded-as-cast}, and \textit{tallied-as-recorded} verifiability~\cite{jonker2013privacy}.

		\noindent\textbf{(5) Dispute-Freeness:} extends the notion of verifiability.
		%		All votes and the tally can be verified by any involved party, hence, the result is indisputable.		
		A dispute-free~\cite{Kiayias2002} voting protocol contains built-in mechanisms eliminating disputes between participants; therefore, anyone can verify whether a participant followed the protocol. 
		Such a scheme has a publicly-verifiable audit trail that contributes to the reliability and trustworthiness of the scheme.
		
		
		\noindent\textbf{(6) Self-Tallying:} once all the votes are cast, any involved party can compute the tally.
%		This property feeds into the public verifiability of the tally.
		Self-tallying systems need to deal with the fairness issues (see (3) above) because the last participant is able to compute the tally even before casting her vote.
		This can be rectified with an additional verifiable dummy vote~\cite{Kiayias2002}.
%		A useful property of privacy-preserving self-tallying protocols is that votes do not need to be unblinded to compute the results of the voting.
		%\IH{put some reference that proposes it}.
		%Another solution is to enforce that participants first commit their votes within a timeout.
		%Although the last participant is still able to compute the final tally before anyone else does, she is no longer able to change her vote.
					
		
		
		\noindent\textbf{(7) Robustness (Fault Tolerance):} the voting protocol is able to recover from faulty (stalling) participants, where faults are publicly visible and verifiable due to dispute-freeness~\cite{Kiayias2002}. 		
		Fault recovery is possible when all the remaining honest participants are involved in the recovery.		
%		Thus, a fault-tolerant protocol ``removes'' participants who quit during the voting.  %  or attempt to vote incorrectly.
		%Non-conforming participants are removed by the protocol without affecting the votes of the remaining participants.
			
		%\noindent\textbf{Receipt-Freeness:} A participant is unable to supply a receipt of her vote after casting the vote.
		%The goal of receipt-freeness is to prevent vote-selling.
		%This property also prevents a post election coercion~\cite{Benaloh1994,Hirt2000}, where a participant may be coerced to reveal her vote.
		%For example, receipt-freeness is a pre-condition for large centralized elections (e.g. national elections).
		%In a distributed setting, receipt-freeness requires an authority to supply additional entropy to the participants (see \autoref{ssec:receiptfreeness}).
		
		\noindent\textbf{(8) Resistance to Serious Failures:}
%		\ih{remove?}
		 Serious failures are defined as situations in which voting results were changed either by a simple error or an adversarial attack. 
		 Such a change may or may not be detected. 
		 If detected in non-resistant systems, it is irreparable without restarting the entire voting~\cite{park2021going}.
%		 \ih{Voting protocols can ensure this property by various means.} 		
	
%		\noindent\textbf{Receipt-indistinguishability:}
%		We define the weaker notion of receipt-freeness aimed at reducing coercion.
%		Receipts of a participants' real and fake votes are available to a post election coercer, but are indistinguishable to the coercer with a tunable probability. 
%		\IH{Please define here.}
%\end{compactitem}




==> sec/protocol.tex <==





\name scheme provides all properties mentioned in \autoref{sec:preliminaries}.
% perfect ballot secrecy, fairness, public verifiability, self-tallying feature, dispute-freeness, resistance to serious failures, and maximizes the voters' privacy (see \autoref{sec:preliminaries}).
Similar to OVN~\cite{McCorrySH17}, \name publishes the full tally at the output and uses homomorphic encryption to achieve privacy of votes and perfect ballot secrecy.
%\IH{I really do not like that I am reffered to appendix at the begining of the paper. Whatever you need should be explained inline here or before. }
%
In detail, we extend the protocol of Hao et al.~\cite{HaoRZ10} to support $k$ choices utilizing the 1-out-of-$k$ proof verification proposed by Kiayias and Yung~\cite{Kiayias2002}, and we accommodate this approach to run on the blockchain. % with Turing-complete smart contracts.
%
Additionally, we extend our protocol to support the robustness, based on Khader et al.~\cite{KhaderSRH12},
which enables the protocol to recover (without a restart) from a number of faulty participants who did not submit their votes.\footnote{This number depends on the blockchain platform's block gas limit and in our evaluation that sets 10M for block gas limit, it is equal to 9 participants.}
As a consequence, robustness increases the resistance of our protocol to serious failures. % (in contrast to OVN).
%Receipt-indistinguishability reduces post-voting coercion attacks. \ih{do we support it? if so, it should be defined in preliminaries.}
%\textbf{Anonymizing identity} thwarts inference attacks on participant voting behavior.



\subsection{Base Variant}
\label{ssec:basicprotocol}
%
\begin{wrapfigure}{t}{0.55\textwidth}
	\centering
	\vspace*{-0.1cm}
	
	\includegraphics[width=\linewidth]{fig/operation-protocol-bw.pdf}
	%	    \vspace{-0.2cm}
	\caption{Basic protocol of \name. The notation $tx(param)_{\mathbb{A}}$ corresponds to a transaction, digitally signed by $\mathbb{A}$'s wallet private key.
		%	    	Timeline of interactions among the $VA$, participants, and smart contract.
		%		Identity verification is carried out off-chain between $VA$ and participant. MPC is carried out by writing and reading transactions to and from the SC respectively. The participant submits blinded vote and proof of its well-formedness to the smart contract. SC verifies the vote and later the tally. 
		%		Events are dispatched signals fired by a smart contract.
	}
	\label{fig:operation-scheme-bw}
	\vspace*{-0.8cm}
\end{wrapfigure}
key ownership verification, enrollment at $SC$), a \textbf{setup} (an agreement on system parameters, submission of ephemeral public keys), \textbf{pre-voting} 
%
The base variant of \name does not involve a fault recovery and is divided into five stages, each describing the actions taken by $P$s and $VA$ in a distributed setting (see \autoref{fig:operation-scheme-bw}).
%\footnote{The notation $tx(param)_{entity}$ corresponds to a blockchain transaction, digitally signed by $entity$'s wallet private key.}
It involves a \textbf{registration} (identity verification, (computation of MPC keys), \textbf{voting} (vote packing, blinding, and verification), and \textbf{tally} phases.
%The non-ephemeral setup parameters are generated once.
%Identity verification is carried out once and the system parameters do not change.
%
All faulty behaviors of $P$s and $VA$ are subject to deposit-based penalties. % (i.e., loss of deposits).
In detail, $P$ who submitted her ephemeral key (in the setup phase) and then has not voted within the timeout will lose the deposit. % while $P$s who voted will get their deposit back. % after voting finishes.
%
To achieve fairness, $VA$ acts as the last $P$ who submits a ``dummy'' vote with her ephemeral private key\footnote{Privacy for a dummy vote is not guaranteed since it is subtracted from the tally.} after all other $P$s cast their vote (or upon the voting timeout expiration). 
%The dummy vote is later subtracted from the final tally by $SC$.



\subsubsection{\textbf{Phase 1 (Registration)}}
%In the first phase, the $VA$ verifies the identity of each participant and the ownership of the participant's private key associated with the blockchain address.
%\noindent\textbf{Identity Verification \& Enrollment}. 
%One way to achieve this is to use a zero-knowledge proof (ZKP) of the private key using Schnorr's signature~\cite{Schnorr1991}, as seen in Kiayias et al.~\cite{Kiayias2002} and Hao et al.~\cite{HaoRZ10}.
%In contrast to previous works, we eliminate the need for ZKP and its verification using blockchain wallet addresses.
%
$VA$ first verifies the identity proof of each $P$.
%\footnote{We assume $VA$ to perform identity proof-verification honestly and neither censor any legitimate $P$ nor register any spoofed $P$.} \ih{we mention in adv model already.}
For decentralized identity management (IDM), the identity proof is represented by the verifiable credentials (VC)~\cite{verifiable-credentails} signed by the issuer, while in a centralized IDM the identity proof is interactively provided by a third-party identity provider (e.g., Google).
First, $VA$ verifies the issuer's signature on the identity proof. 
Next, $VA$ challenges $P$ to prove (using her VC) that she is indeed the owner of the identity.
Further, each $P$ creates her blockchain wallet address (i.e., the blockchain public key (PK)) and provides it to $VA$.
% 
The $VA$ locally stores a bijective mapping between a $P$'s identity and her wallet address.\footnote{Note that the address of $P$ must not be part of identity proof to preclude $VA$ from owning an indisputable proof of identity to blockchain address mapping (see \autoref{sec:blockchain-specific-issues}).} 
%To verify ownership of a private key linked to a submitted address, $VA$ performs an off-chain challenge-response-based verification with each $P$. \ih{this is too detailed and it is not necessary.}
Next, $VA$ enrolls all verified $P$s by sending their wallet addresses to $SC$.
%We remark that $VA$ is unable to provide indisputable proof of the identity-PK mapping of $P$s to the public since PK is freshly generated and is not presented in the identity proof.

%$P$s never supply it to $VA$ and the communication between the $VA$ and the $P$s during the registration is carried out through e.g., HTTPS protocol, which does not require clients to have registered PKs in X.509 PKI in contrast to $VA$ (see \autoref{sec:discussion}).


%\begin{compactitem}
\subsubsection{\textbf{Phase 2 (Setup)}}
	$P$s agree on system parameters that are universal to voting -- the parameters for voting are publicly visible on $SC$ (deployed by $VA$ in a transaction).
	Therefore, any $P$ may verify these parameters before joining the protocol.
	Note the deployment transaction also contains the specification of timeouts for all further phases of the protocol as well as deposit-based penalties for misbehavior of $VA$ and $P$s.
	The parameters for voting are set as follows:

\setlength{\parskip}{5pt} \setlength{\itemsep}{5pt}
\begin{compactenum}[$\;$]
	\item[1)] $VA$ selects a common generator $g\in \mathbb{F}_p^*$. 
	The value of $p$ is chosen to be a safe prime, i.e., $p=2\cdot  q +1$, where $q$ is a prime. 
	A safe prime is chosen to ensure the multiplicative group of order  $p - 1 = 2\cdot q$, which has no small subgroups that are trivial to detect.\footnote{We use modular exponentiation by repeated squaring to compute $g^x$ $mod$ $p$, which has a time complexity of $\mathcal{O}$(($log$ $x$)$\cdot (log^2$ $p$))~\cite{Koblitz}. } % Note the increase in time complexity w.r.t. the exponent is logarithmic.
	%
	Let $n < p - 1$.	
	\item[2)] Any participant $P_i$ is later permitted to submit a vote $\{v_i ~|~ i\in \{1,2,...,k\}\}$ for one of $k$ choices. This is achieved by selecting $k$ independent generators $\{f_1,...,f_k\}$  in $\mathbb{F}_p^*$ (one for each choice).
	%
	These generators for choices should meet a property described by Hao et al.~\cite{HaoRZ10} to preclude having two different valid tallies that fit \autoref{eqn:eq3}:
	\begin{eqnarray}
		f_i = 
		\begin{cases}
		g^{2^0}       & \quad \text{for choice 1},\\
		g^{2^m}       & \quad \text{for choice 2},\\
		\quad \quad \quad \cdots \\
		g^{2^{(k-1)m}} & \quad \text{for choice k},
		\end{cases}
	\end{eqnarray}
	where $m$ is the smallest integer such that $2^m > n$ (the number of participants).		
\end{compactenum}

%\sarad{does equation 1 guarantee that the generators will not clash?.}\ih{Yes, as per Hao paper.}
	
	\noindent\textbf{Ephemeral Key Generation \& Committing to Vote.}
	Each $P_i$ creates her ephemeral private key as a random number $x_i\in_{R} \mathbb{F}_p^*$ and ephemeral public key as $g^{x_i}$.
	Each $P_i$ sends her ephemeral public key to $SC$ in a transaction signed by her wallet, thereby, committing to submit a vote later.\footnote{Note that in contrast to OVN~\cite{McCorrySH17} (based on the idea from~\cite{HaoRZ10}), we do not require $P_i$ to submit ZKP of knowledge of $x_i$ to $SC$ since $P_i$ may only lose by submitting $g^{x_i}$ to which she does not know $x_i$ (i.e., losing a chance to vote and the deposit). 
	}
	Furthermore, $P_i$ sends a deposit in this transaction, which can be retrieved back after the end of voting.
	However, if $P_i$ does not vote within a timeout (or does not participate in a fault recovery (see \autoref{sec:faulttolerance})), the deposit is lost, and it is split to the remaining involved parties.
	$P$s who do not submit their ephemeral keys in this stage are indicating that they do not intend to vote; the protocol continues without them and they are not subject to penalties.		
	Finally, each $P$ obtains (from $SC$) the ephemeral public keys of all other verified $P$s who have committed to voting.
	%
	Note that ephemeral keys are one-time keys, and thus can be used only within one run of the protocol to ensure privacy of votes (other runs require fresh ephemeral keys). % of the protocol.
%	If $P$ were to vote in a different instance of e-voting, she would generate new ephemeral keys.


\subsubsection{\textbf{Phase 3 (Pre-Voting)}}
This phase represents multiparty computation (MPC), which is run to synchronize the keys among all $P$s and achieve the \textit{self-tallying} property.
However, no direct interaction among $P$s is required since all ephemeral public keys are  published at $SC$. The MPC keys are computed by $SC$, when $VA$ triggers the compute operation via a transaction.
%
The $SC$ computes and stores the MPC key for each $P$ as follows:
	\begin{equation}
	\label{eqn:eq1}
	h=g^{y_i}=\prod\limits_{j=1}^{i-1} g^{x_j}/\prod\limits_{j=i+1}^{n} g^{x_j},
	\end{equation}
	where $y_i=\sum_{j<i}x_j- \sum_{j>i}x_j$
	and
	$\sum_{i}x_i y_i=0$ (see Hao et al.~\cite{HaoRZ10} for the proof).
	Since $y_i$ is derived from the private ephemeral keys of all other $P$s it is secret. % \ih{not relevant here}
	%
	While anyone can compute $g^{y_i}$, to reveal $y_i$, all $P$s $\setminus $ $P_i$ must either collude or solve the DLP for \autoref{eqn:eq1}.\footnote{Note that this DLP was already computed for 795-bit long safe prime in 2019~\cite{integer-dlp-2019}; the computation took $\sim3100$ core-years, using Intel Xeon Gold 6130 (2.1GHz) CPUs.} 
	%Since each $P_i$ can obtain $g^{y_i}$ of all $P$s, she alone can compute (ephemeral blinding key) $g^{x_i y_i}$ using her private key $x_i$.
%	Each pair of $P$s share exactly one slice of the ephemeral blinding key; this counter-party property is utilized in the fault recovery mechanism (see \autoref{sec:faulttolerance}).
	%
	As the corollary of \autoref{eqn:eq1}, the protocol preserves vote privacy if there are at least 3 $P$s with at least 2 honest (see the proof in \autoref{sec:appendixvoteorivacy}). 
	

%%
%\footnote{Note that this DLP was already computed for 795-bit long safe prime in 2019~\cite{integer-dlp-2019}; the computation took $\sim3100$ core-years, using Intel Xeon Gold 6130 (2.1GHz) CPUs.} 
%Since each $P_i$ can obtain $g^{y_i}$ of all $P$s, she alone can compute (ephemeral blinding key) $g^{x_i y_i}$ using her private key $x_i$.

\begin{figure}[t]
	\begin{center}
		\scriptsize
		\vspace{-0.3cm}
		\fbox{
			\begin{protocolm}{2}						
				\participants{\underline{Participant $P_i$}}{\underline{Smart Contract}}
				\participants{($~h\leftarrow g^{y_i},~ v_i$)}{($~h\leftarrow g^{y_i}$)}
				\hline	
				& &\\		
				%				\text{Generates~vote~choice~of} \\
				Select~v_i\in\{1,...,k\}, & & \\	 				
				Use~choice~generators~\\
				f_l\in\{f_1,...,f_k\}\subseteq\mathbb{F}_p^*,\\			
				%Publish:~B_i\leftarrow h^{x_i}{f_l}\\
				Publish~ x\leftarrow g^{x_i} && 	\\
				Publish~ B_i\leftarrow h^{x_i}{f_l} & & \\
				
				%h\leftarrow g^{y_i} && h\leftarrow g^{y_i}(Computed~in~Equation~ \ref{eqn:eq1})	\\
				
				w\in_{R} \mathbb{F}_p^*\\
				%a_{v_j}\leftarrow g^{w} \\
				%b_{v_j}\leftarrow h^{w} \\
				
				
				\forall l\in \{1,..,k\}\setminus {v_i}:\\
				
				\quad 1.~r_l,d_l\in_{R} \mathbb{F}_p^* \\
				\quad 2.~a_l\leftarrow x^{-d_l}g^{r_l}\\ 				
				\quad 3.~b_l\leftarrow h^{r_l}(\frac{B_i}{f_l})^{-d_l} \\
				
				
				
				for\enspace {v_i}:\\
				
				\quad 1.~a_{v_i}\leftarrow g^{w}\\
				\quad 2.~b_{v_i}\leftarrow h^{w} \\
				%&\stackrel{\forall l: \{a_l\},\{b_l\}}{\xrightarrow{\hspace*{4.5cm}}}&\\
				\hdashline
				c\gets\Hzk(\{ \{a_l\},\{b_l\} \}_{l})\\
				\hdashline
				%&\sends{\forall l: \{a_l\},\{b_l\}}&\\
				%&\receives{c}&c\leftarrow \mathbb{Z}_q  \\
				
				for\enspace {v_i}:\\
				
				%\quad 1.~d_{v_i}\leftarrow c \bigoplus_{l\neq{v_i}}d_l\\
				\quad 1.~d_{v_i}\leftarrow \sum_{l\neq{v_i}}d_l\\
				\quad 2.~d_{v_i}\leftarrow c - d_{v_i}\\
				
				\quad 3.~r_{v_i}\leftarrow w+x_id_{v_i} \\			
				\quad 4.~q\leftarrow p-1\\
				\quad 5.~{r_{v_i}\leftarrow r_{v_i}\mod{q}}\\			
				
				
				%&\stackrel{\forall l:\{r_l\},\{d_l\}}{\xrightarrow{\hspace*{4.5cm}}}
				&\sends{\forall l: \{a_l\}, \{b_l\}, \{r_l\},\{d_l\}}
				&\\
				
				& &\Psi \gets \{\forall l: \{a_l\},\{b_l\}\}  \\
				&& c \gets\Hzk(\Psi)\\
				
				%& &d_{sum}\leftarrow\sum_{l}d_l~mod~p-1\\
				& &\sum_{l} d_{l} \stackrel{?}{=} c\\
				
				&& \forall l\in \{1,..,k\}\\
				%&& && x^{{r_{v_j}}}\stackrel{?}{=}{a_{v_j}}x^{d_{v_j}}\\
				
				
				&&\quad 1.~g^{r_l}\stackrel{?}{=}{a_l}x^{d_l}\\
				&&\quad 2.~h^{r_l}\stackrel{?}{=}{b_l}(\frac{B_i}{{f_l}})^{d_l}\\
				%h^{r_{v_j}}\stackrel{?}{=}{b_{v_j}}(B_i/{f_l})^{d_{v_j}}\\			
			\end{protocolm}
		}
	\end{center}
	\vspace{-0.35cm}
	\caption{Zero knowledge proof of set membership for 1-out-of-$k$ choices. }
	\label{fig:ZKPMultiCandidate}
	\vspace{-0.5cm}
\end{figure}	

\subsubsection{\textbf{Phase 4 (Voting)}}
In this phase, each $P_i$  blinds and submits her
vote to $SC$.
These steps must ensure the recoverability of the tally, vote privacy, and well-formedness of the vote.
%Taking into consideration the structural similarity with the anonymous veto protocol used in \autoref{ssec:votechange}, 
%We adopt a DLP-based cryptosystem over homomorphic encryption (such as Pallier cryptosystem~\cite{Pascal99}) \ih{is it correct also for ECC implementation?}.
%This is mainly due to the easier deployability of DLP-based solutions at a smart contract platform (see~\autoref{sec:implementation}).
%zero knowledge set membership proofs for 1-out-of-$k$ candidates are presented in Kiayias et al.~\cite{Kiayias2002} and Baudron et al. ~\cite{Baudron2001}.
Vote privacy is achieved by multiplying the $P_i$'s blinding key with her vote choice.
The blinded vote of the participant $P_i$ is
\begin{equation}
\label{eqn:eq2}
B_i=\begin{cases}
g^{x_iy_i}f_1 & \text{if $P_i$ votes for choice 1},\\
g^{x_iy_i}f_2 & \text{if $P_i$ votes for choice 2},\\
~~~~~~~~~~~~~...\\
g^{x_iy_i}f_k & \text{if $P_i$ votes for choice \textit{k}.}
\end{cases}
\end{equation}
The $P$ sends her choice
%homomorphically encrypted (sarad: there is no homomorphic encryption here, its just blinded. the homomorphsim property is used for tallying, where the votes are added up in the exponent.) 
 within a blinded vote along with a  1-out-of-$k$ non-interactive zero-knowledge (NIZK) proof of set membership to $SC$.
We modified the approach proposed in Kiayias et al.~\cite{Kiayias2002} to the form used by Hao et al.~\cite{HaoRZ10}, which is convenient for practical deployment on existing smart contract platforms.
The verification of set membership using this protocol is depicted in \autoref{fig:ZKPMultiCandidate}, where $P_i$ is a prover and $SC$ is the verifier.
Hence, $SC$ verifies the correctness of the proof and then stores the blinded vote.
%
In this stage, it is important to ensure that no re-voting is possible, which is to avoid any inference about the final vote of $P$ in the case she would change her vote choice during the voting stage.
Such a re-voting logic can be enforced by $SC$, while user interface of the $P$ should also not allow re-voting.
Moreover, to ensure fairness, $VA$ acts as the last $P$ who submits a dummy vote together with her ephemeral private key.
 
	

\subsubsection{\textbf{Phase~5~(Tally)}}
When the voting finishes (i.e., voting timeout expires or all $P$s and $VA$ cast their votes), the tally of votes received for each of $k$ choices is computed off-chain by any party and then submitted to $SC$.
When $SC$ receives the tally, it verifies whether \autoref{eqn:eq3} holds, subtracts a dummy vote of $VA$, and notifies all $P$s about the result. % of the tally. 
%
The tally is represented by vote counts $ct_i,\forall i\in\{1,...,k\}$ of each choice, which are computed using an exhaustive search fitting 
%
\begin{equation}
\label{eqn:eq3}
\prod\limits_{i=1}^{n}B_i=
\prod\limits_{i=1}^{n}g^{x_iy_i}f=
g^{\sum_{i}x_i y_i}f=
{f_1}^{ct_1}{f_2}^{ct_2}...{f_k}^{ct_k}.
\end{equation}
%Note that $g^{\sum_{i}x_i y_i}=1$ since $\sum_{i}x_i y_i=0$. \ih{Looks irrelevant.}
The maximum number of attempts is bounded by combinations with repetitions to ${n+k-1}\choose{k}$.
%\IH{This could be optimized to permutation of a few Stirling numbers of the second order in the next version.}
%
Although the exhaustive search of 1-out-of-$k$ voting is more computationally demanding in contrast to 1-out-of-2 voting~\cite{McCorrySH17},~\cite{HaoRZ10}, this process can be heavily parallelized. 
See time measurements in \autoref{sec:tally-exps}.
%
%Note that Kiayias and Yung~\cite{Kiayias2002} propose to apply baby-step giant-step method (proposed by Shanks) to reduce the time complexity of the exhaustive search to $\mathcal{O}(\sqrt{n}^{k-1})$ attempts.
%However, we argue that it is not trivial since baby-step giant-step method is intended to compute a single DLP while \autoref{eqn:eq3} contains multiple DLP problems as part of the product.
%\sarad{i commented it out because i doubt what i told is correct. it is still multi-dlp even for 2 candidates, right? }
%Note this text is unrelated to the security of the voting protocol.

%Moreover, if a high number of the $P$s and/or the vote choices would cause a longer computation time than is acceptable (even in the case of parallelization), the time complexity can be further reduced by the to $\mathcal{O}(\sqrt{n}^{k-1})$ attempts~\cite{Kiayias2002}.

%\sarad{the question is how? Shanks solves the discrete problem, we need to solve the multi-dlp. let us not give away our ideas until we build it ourselves. i prefer we not say this, as it is currently only speculation. Either we show how it works or avoid saying it.}


==> sec/relatedwork.tex <==
In this section, we briefly survey existing paradigms in e-voting and describe a few blockchain-based e-voting approaches. 
In particular, we focus on remote voting approaches (with sufficient specification), which we compare in \autoref{tab:comparison}. % in terms of voting and other  features. 


\myparagraph{\textbf{E-Voting Paradigms}}
Utilization of mix-nets that shuffle the votes to break the map between $P$s and their votes was proposed by Chaum~\cite{Chaum1981}.
%
Benaloh and Fischer~\cite{Cohen1985} were among the first who showed a paradigm shift from anonymizing $P$s to providing privacy of the vote.
Cramer et al.~\cite{cgs97} present a model where all votes are sent to a single combiner, utilizing homomorphic properties of the ElGamal cryptosystem~\cite{Elgamal85}. % to compute the encrypted tally.
%The tally itself is computed by solving DLP, whose complexity is proportional to the number of $P$s.
Using bulletin board and zero-knowledge proofs allow their protocol to be universally verifiable.
%
The work of Kiayias and Yung~\cite{Kiayias2002} converts this scheme into a self-tallying combiner supporting 1-out-of-2 choices; further, the authors outline an extension of their base protocol to support 1-out-of-k choices.
Hao et al.~\cite{HaoRZ10} improve upon the self-tallying protocol by proposing a simple general-purpose two-round voting protocol for 1-out-of-2 choices with low bandwidth requirements and computational costs.
%However, Hao et al.~\cite{HaoRZ10} limit the number of choices to two.
%
Khader et al.~\cite{KhaderSRH12} take it a step further by adding fairness and  robustness properties.
%Furthermore,  they mostly rely on a centralized bulletin board, which introduces a single point of failure.
%In contrast to the above schemes, our protocol uses a decentralized and immutable bulletin board represented by the blockchain.
%
Groth~\cite{Groth2004} introduces an anonymous broadcast channel with perfect message secrecy leveraged in his voting protocol that is simpler and more efficient than~\cite{Kiayias2002}. 
However, it requires sequential voting, where each voter has to download a fresh state of the bulletin board before voting.
%
Zagorski et al.~\cite{zagorski2013remotegrity} propose Remotegrity that is based on Scanintegrity~\cite{chaum2008scantegrity} ballots mailed to voters, allowing them remotely vote and verify that their ballots were correctly posted to the bulletin board and at the same time providing protection against malware in clients.
%
Another direction (e.g.,~\cite{kusters2020ordinos,huber2022kryvos}) focuses on the tally-hiding~\cite{benaloh1986improving,hevia2002electronic} property that is suitable for some use cases requiring to reveal only the best $m$ candidates.

\vspace{-0.2cm}
\myparagraph{\textbf{Location}}
Voting systems can be classified by the physical location where the vote is cast.
Some schemes allow $P$s to submit a vote from their devices (i.e., \textit{remote voting}), e.g.,~\cite{KiayiasAdder06},~\cite{Adida08},~\cite{zagorski2013remotegrity}, and blockchain-based~\cite{followMyVote-blockchain-simple-voting},~\cite{tivi-blockchain-simple-voting}. 
%
Others systems require voting to be carried out at a designated site (a.k.a., \textit{supervised voting}), e.g.,~\cite{chaum2008scantegrity},~\cite{Rui2012},~\cite{Sandler08},~\cite{Bell2013},~\cite{ShahandashtiH16}, and blockchain-based~\cite{soud2020trustvote},~\cite{hjalmarsson2018blockchain},~\cite{agora2018}.


%\myparagraph{\textbf{Location}}
%E-voting systems can be classified by the physical location where the vote is submitted.
%Some schemes allow $P$s to submit a vote from their computing device (i.e., \textit{remote voting}), e.g., Adder~\cite{KiayiasAdder06}, Helios~\cite{Adida08}, Remotegrity~\cite{Filip2013}, \ih{as well as blockchain-based Follow My Vote~\cite{followMyVote-blockchain-simple-voting}}. 
%%
%Others systems require voting to be carried out at a designated site (a.k.a., \textit{supervised voting}), e.g., MarkPledge~\cite{Rui2012}, VoteBox~\cite{Sandler08}, Star-Vote~\cite{Bell2013}, DRE-ip~\cite{ShahandashtiH16}, \ih{as well as blockchain-based proposals TrustVote~\cite{soud2020trustvote} Hj{\'a}lmarsson et al.~\cite{hjalmarsson2018blockchain}, ...}.
%
%We emphasize that our protocol is suitable for vote submission to use the participants' devices and requires no additional infrastructure.
%Electronic voting is an actively researched topic and one of the earliest work in this direction is known to be from Chaum~\cite{Chaum1981}.
%The current research space, based on the structure and responsibilities of the parties involved in the electoral process, is split into two directions; ly, de-centralized and centralized e-voting.
%In a de-centralized setting, a multiparty computation round is run between the participants~\cite{Kiayias2002,Groth2004,HaoRZ10}, whereas in a centralized setting, an authority runs the election~\cite{RyanBHSX09}.
%In a de-centralized setting, the focus is on security and a minimal amount of trust is assumed.
%In a centralized setting, the authority is assumed to be trustworthy and they play a bigger role in the election.
%The focus is on usability, scalability and robustness (fault tolerance).
%Their centralized nature makes it robust and suitable for large elections.

\vspace{-0.3cm}
\subsection{Blockchain-Based E-Voting}
\vspace{-0.3cm}
We extend the categorization of (remote) blockchain-based voting systems~\cite{yu2018platform} in the following, while we focus on smart contract-based systems.


%\ih{also check -- Kryvos \url{https://dl.acm.org/doi/abs/10.1145/3548606.3560701} (likely provides only the winner without tally, so use it as an example.). Also, it is non-blockchain-based.}

%\ih{Sarad, please include Provotum~\cite{killerprovotum}, which is very related. Maybe also check their other paper~\cite{killer-sac}}
%\ih{Another issue that Christian Killer reported is :"Matile et al. has privacy of votes \& also source code is available"}

%Various blockchain-based e-voting systems have been proposed in recent years~\cite{McCorrySH17,EPRINT:PanRoy18,icissp:DMMM18,ICBC:MRSS19}.
%In particular, 
%%


\vspace{-0.3cm}
\myparagraph{\textbf{(a) Voting Systems Using Smart Contracts}}
%
McCorry et al.~\cite{McCorrySH17} proposed OVN, a self-tallying voting protocol (basing on~\cite{HaoRZ10}) that provides vote privacy and supports two vote choices.
OVN is implemented as Ethereum $SC$ and is suitable for boardroom voting. 
It does not provide robustness and expensive tally computation is made by $SC$. 
In contrast, \name only verifies the tally in $SC$, while it is computed off-chain.
%
Similar approach basing on~\cite{HaoRZ10} was proposed by Li et al.~\cite{Li2020}, who further provided robustness from~\cite{KhaderSRH12}.
%
Seifelnasr et al.~\cite{DBLP:conf/fc/SeifelnasrGY20} aimed to increase the scalability of OVN by off-chaining tally computation and registration at $VA$ in a verifiable way. 
Due to the higher costs imposed by storing data on $SC$, they compute the Merkle tree of voter identities and store only its root hash at $SC$. 
Their approach requires only a single honest $P$ to maintain the protocol's security by enabling her to dispute the incorrect tally submitted to $SC$.
The scalability technique proposed in this paper is orthogonal to us, and it can be combined with our techniques (see \autoref{ssec:scalability-improvements}) to achieve higher savings of the on-chain costs.
%
%
%The authors do not perform verification of off-chained computations by $SC$, but instead, assume at least one honest voter who can contend the authority's claimed result if it was not computed correctly.\ih{$=>$ some property not met?}
%
%%%%%%%
%
Yu et al.~\cite{yu2018platform} employ ring signature to ensure that the ballot is from one of the valid choices, and they achieve scalability by linkable ring signature key accumulation. % algorithms.
Their approach provides receipt-freeness 
%(under the assumption that $VA$ does not reveal the Paillier system secrets to anyone), 
under the assumption of trusted $VA$.
However, we argue that this property is useless when remaining coercion-prone (typical to remote voting).
Moreover, due to receipt-freeness, this approach does not provide E2E verifiability (i.e., cast-as-intended and recorded-as-cast). 
%
Killer et al.~\cite{killerprovotum} present an E2E verifiable remote voting scheme with two vote choices. % based on a public permissioned blockchain. 
The authors employ threshold cryptography for achieving robustness using a scheme similar to Shamir secret sharing. 
%\ih{Sarad: are you sure about FT? Also why it does not provide self tallying? Sarad: self-tallying: the votes need to be decrypted by n-of-n autorities; fault-recovery: it is inherent to Pailler cryptosystem since to tally the votes are just summed (faulty/missing ones are not summed)}
However, it supports only integers up to a 256 bits (i.e., a size of the EVM word), which is far below a minimal secure length.
%
%Our implementation is  tailored for a public blockchain (i.e., we count costs) and the costs to carry out additional SSS is a bottleneck we avoid.
% 
%From Provotup paper:
%Results Phase: Once all Sealers have submitted the
%decrypted shares, and the ballot SC persists them, the VA
%triggers the final decryption step. The ballot SC combines the
%decrypted shares dsealeri
%and generates the decrypted result
%of all votes. The result is stored in the ballot SC, and anyone
%can verify the result by combining the decrypted shares.
%
%ih{does it has fault tolerance then? Also, what if a threshold of sealers (consensus nodes) would not submit the shares?}
%
Matile et al.~\cite{ICBC:MRSS19} proposed a voting system providing cast-as-intended (but neither E2E nor universal) verifiability. %enabling any voter to verify that her encrypted vote represents the decision she made.
Their system uses ElGamal encryption based on DLP with integers modulo $p$. 
Since existing blockchains support natively only up to 256-bit security for this DLP, the authors create the custom blockchain with sufficient security. 
%
%In open-audit voting schemes, a participant may choose to either audit or submit her vote.
%If she chooses to audit~\cite{BenalohAudit2006}, the vote needs to be re-submitted.
%A participant is allowed to audit her vote an arbitrary number of times before re-submission.\ih{I do not understand the reason why?}
%Here, audit plays an important role in reducing the chances that an unintended vote was submitted.
%They are used in web based voting applications such as Helios~\cite{Adida08}.
%
Dagher et al.~\cite{icissp:DMMM18} proposed BroncoVote, a voting system that preserves vote privacy by homomorphic encryption (i.e., Paillier cryptosystem) -- the authors do not provide full deployment on the blockchain but off-chain all cryptographic operations to a trusted server (without verifiability), which introduces a vulnerability. % of single-point-of-failure. %while keeping the voting system transparent.
%Besises, security of cryptographic operations with IA in BroncoVote use only native 256-bit long numbers in Solidy, which does not provide a suffient security level.
%In a nutshell, BroncoVote implements a university-scaled voting framework that utilizes Ethereum's blockchain and smart contracts to achieve voter administration and auditable voting records.
%
Kostal et al.~\cite{kovst2019blockchain} propose voting system, in which $VA$ serves as a trusted key generator that distributes private keys for homomorphic encryption to voters, which enables them to resolve robustness issues at the cost of putting a strong trust into $VA$.
This, however, enables $VA$ to sabotage voting or decrypt the tally before voting finishes. 
%\ih{check this with Kiko.}

%Zhang et al.~\cite{Zhang18} allows solo cheating, which however, can be detected by honest peers.
%Privacy is achieved by encryption by public keys of blockchain peers!


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Weak ones from here:
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%Literature also contains conceptual approaches. % that were not evaluated or analyzed in terms of voting features and security.
%
%\ih{bookmark}

%Panja and Roy~\cite{EPRINT:PanRoy18} present an auditable local (DRE) voting system. 
%%which describes voting processes and components of a supervised Internet voting system that is audit and verification capable.
%The authors achieve auditability and verifiability by the utilization of the blockchain and voter-verified audit trail.


%three main roles: vote publisher; key authority (KA); and voter.
%The vote publisher has to know all cipher keys before publishing the smart contract.
%The key authority creates and distributes all cipher keys to a voter and vote publisher.
%The close collaboration between the vote publisher and the key authority is required. 
%This KA serves vote publisher and voter to obtain public key for homomorphic encryption and a key to access the votes.
%
%The smart contract has to contain
%the public key of the homomorphic encryption to make the
%encrypted results of the elections. The private key is stored
%separately and is used to see results after the voting ends. This
%key can be distributed to multiple parties which are responsible
%for voting evaluation. 



\vspace{-0.3cm}
\myparagraph{\textbf{(b) Voting Systems Using Cryptocurrency}}
%
Zhao and Chan~\cite{zhao2015vote} propose a privacy-preserving voting system with 1-out-2 choices based on Bitcoin, which uses a lottery-based approach with an off-chain distribution of voters' secret random numbers with their ZKPs.
%in which ballots do not need to be encrypted/decrypted due to lottery-based protocol .
%Random numbers enable to hide the ballot, and they that are distributed via ZKP.
The authors use deposits incentivizing $P$s to comply with the protocol; however, a malicious $P$ can sabotage the voting by refusing to vote or vote in a different order than required. % => not providing fault tolerance and thus resistance to serious failures.  % \ih{it seems to have similar properties than \cite{Groth2004}} 
%
Tarasov and Tewari~\cite{tarasov2017internet} proposed a conceptual voting system based on Zcash. %without altering the inner working of Zcash protocol. 
The voter's anonymity (and thus privacy of vote) is ensured by the z-address that preserve unlinkability. 
The correctness of the voting is guaranteed by the trusted $VA$ and the candidates. 
%In this system, the authority, who manages the Zcash and voter status database should be trusted. 
If $VA$ is compromised, double-voting or tracing the source of the ballot (violating privacy) is possible.
%The protocol allows misbehaving of candidates, which can be only detected by trusted $VA$.
%\ih{They have really cool related work!}
%
Liu and Wang~\cite{liu2017voting} propose a conceptual voting approach that is based on blind signatures with 2 vote choices. 
They utilize blockchain only for (auditable) sending of the messages among parties.
However, despite using blind signatures, $P$s send their vote to blockchain in plain-text, thus the authors recommend anonymization services.
%It assumes trusted $VA$ and inspectors that oversee $VA$.


\vspace{-0.3cm}
\myparagraph{\textbf{(c) Commercial Voting Systems with Ballot Box}}
%
FollowMyVote~\cite{followMyVote-blockchain-simple-voting} and Tivi~\cite{tivi-blockchain-simple-voting} use blockchain for recording of plain text votes into a \textit{ballot box}, where privacy of votes relies only on the assumption that a public key of $P$ cannot be linked to her identity, which is not resistant to $\mathcal{A}$.
%
NetVote~\cite{netvote2018} is the solution addressing privacy by trusting $VA$ to reveal the encryption key of ballots after the election ends. 
However, $VA$ can refuse to reveal the key or reveal it before the voting ends.
In NetVote, ballot boxes correspond to electoral districts, each of them having its smart contract.
Each such smart contract includes a list of votes, also represented by
smart contracts, which, however, is an expensive solution.
%
%These approaches are without any in-depth specification and security \& analysis.
%\ih{TODO -  BitCongress's Whitepaper (Rockwell, 2015) }

%\ih{Other examples: Some examples active at the time of this writing, summer 2018, include Follow My Vote https://followmyvote.com/, Polys https://polys.me/, SecureVote	https://secure.vote/, VoteWatcher http://votewatcher.com/, Agora https://agora.vote, e-Vox http://e-vox.org/, TIVI https://tivi.io/, Boul´e https://www.boule.one/, Democracy.Earth https://www.democracy.earth/, Voatz https://voatz.com/, Coalichain https://www.coalichain.io/, etc.}


% Helios
%is the first online, open-audit voting protocol. Helios’
%first priority is data integrity; then it addresses voter
%privacy. To ensure data integrity, any observer may
%audit the election process at any time during the election. Although an individual's name is initially posted
%along with the individual’s encrypted vote, after the
%election closes, the votes are shuffled and then the
%result is computed. Helios claims to be the optimal
%voting system for small groups where coercion is unlikely but private voting is necessary 
%Although Helios maintains data integrity, voter privacy is not preserved to the utmost.


%\ih{Discuss missing coercion resistance of remote voting and possible transformation of \name to supervised system.}

\renewcommand{\arraystretch}{1.1}
%\setlength{\tabcolsep}{0.5cm}
\setlength{\tabcolsep}{7.0pt}
\begin{table*}[t]
	\vspace{-0.4cm}
	\centering
	\scriptsize
	
	\begin{tabular}[t]  {l c c c c c c c c c c}
		%		{p{2.5cm} p{1cm} p{1cm} p{1cm}  p{1cm} p{1cm} p{1cm}}
		%\cline{2-11}
		\toprule
		\textbf{\specialcell{Approach\\}} & \trot{\textbf{Privacy of Votes}} & \trot{\textbf{\specialcell{Perfect Ballot Secrecy}}} & \trot{\textbf{Fairness}}  & \trot{\textbf{Self-Tallying}} & \trot{\textbf{Robustness}} &  \trot{\textbf{\specialcell{ Uses Blockchain}}} & \trot{\textbf{Uni. Verifiability}} &  \trot{\textbf{E2E Verifiability}}  & \trot{\textbf{Open Source}} & \trot{\textbf{Choices}}\\
		\toprule
		
		Hao et al.~\cite{HaoRZ10} & \hfil\cmark & \hfil\cmark & \hfil\xmark & \hfil\cmark & \hfil\xmark & \hfil\xmark  & \hfil\cmark & \hfil\cmark  & \hfil\xmark &  \hfil $2$\\
		
		Khader et.~\cite{KhaderSRH12} & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark  & \hfil\xmark  & \hfil\cmark & \hfil\cmark & \hfil\xmark & \hfil $2$\\
		
		Kiayias and Yung~\cite{Kiayias2002} & \hfil\cmark & \hfil\cmark & \hfil\cmark  & \hfil\cmark & \hfil\cmark & \hfil\xmark  & \hfil\cmark & \hfil\cmark  & \hfil\xmark & \hfil $2 / k$\\
		
		McCorry et.~\cite{McCorrySH17} (OVN) & \hfil\cmark & \hfil\cmark & \hfil\cmark  & \hfil\cmark & \hfil\xmark &  \hfil\cmark & \hfil\cmark & \hfil\cmark  & \hfil\cmark & \hfil $2$\\
		
		Seifelnasr et al.~\cite{DBLP:conf/fc/SeifelnasrGY20} (sOVN) & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\xmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil $2$  \\								
		
		
		Li et al.~\cite{Li2020} & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark &  \hfil \cmark  & \hfil\cmark & \hfil\cmark & \hfil\xmark & \hfil $2$\\
		% It contains pretty simple security analysis, which we can do as well - https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9031381
		
%		Zhang et al.~\cite{Zhang18} & \hfil\cmark & \hfil\xmark & \hfil\xmark & \hfil\xmark & \hfil\cmark &  \hfil\cmark  & \hfil\cmark & ? & \hfil\xmark & \hfil $k$\\ \ih{This is too weak to be included. Even privacy relying on trusted blockchain peers, who can reveal vote choice of a participant.}
		
		Baudron et al.~\cite{Baudron2001} & \hfil\cmark & \hfil\xmark & \hfil\xmark & \hfil\xmark & \hfil\cmark &  \hfil\xmark & \hfil\cmark & \xmark & \hfil\xmark & \hfil $k$\\ %\ih{seems interesting to look into later}
		
		Groth~\cite{Groth2004} & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\xmark & \hfil\xmark  & \hfil\cmark & \cmark & \hfil\xmark & \hfil $k$\\
		
		Adida~\cite{Adida08} (Helios) & \hfil\cmark$^*$  & \hfil\xmark & \hfil\xmark & \hfil\xmark & \hfil\cmark & \hfil\xmark & \hfil\cmark & \cmark & \hfil\cmark & \hfil $k$  \\
		
		Matile et al.~\cite{ICBC:MRSS19} (CaIV) & \hfil\cmark & \hfil\xmark & \hfil\xmark & \hfil\xmark & \hfil\cmark & \hfil\cmark & \hfil\xmark & \hfil\xmark & \hfil\cmark &  \hfil $k$\\
		
		Killer~\cite{killerprovotum} (Provotum) & \hfil \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark & \hfil \cmark & $2$ \\			
		
%		\ih{Panja and Roy}~\cite{EPRINT:PanRoy18} & \hfil ? & ? & ? & ? & ? & ? & ? & ? & ? & \hfil ?  \\  %\ih{Does not belong here since it is local (supervised)
		
		Dagher et al.~\cite{icissp:DMMM18} (BroncoVote)			 & \hfil \cmark & \cmark$^*$ & \cmark$^*$ & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \hfil $k$  \\
		

		Kostal et al.~\cite{kovst2019blockchain} & \cmark$^*$  &  \cmark$^*$ & \xmark & \cmark & \cmark$^*$ & \cmark & \cmark  & \cmark & \xmark & $k$  \\
		
		
		%\ih{Kiayias et al.}~\cite{KiayiasAdder06}		 & \hfil ? & ? & ? & ? & ? & ?  & ? & ? & \hfil ?  \\
		
%		Shahandashti and Hao~\cite{ShahandashtiH16} (DRE-ip)		 & \hfil\cmark &\hfil\xmark  & \hfill\xmark &\hfill\xmark  &\hfill\cmark & \hfill\xmark & ? & \hfill\cmark & \hfil\xmark & \hfil $k$  \\ %\ih{Does not belong here since it is local (supervised)
		
		Zagorski et al.~\cite{zagorski2013remotegrity} (Remotegrity)		 & \cmark$^*$ & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & $k$  \\
		
%		Rui and Ribeiro~\cite{Rui2012}		 	& \hfil\cmark  & \hfil\xmark & \hfil\xmark & \hfil\xmark  & \hfil\cmark & \hfil\xmark &  \hfil\cmark & ? & \hfil\xmark & $k$  \\ \\ %\ih{Does not belong here since it is local (supervised)
		
%		Sandler et al.~\cite{Sandler08} (VoteBox)	& \hfil\cmark  & \hfil\xmark & \hfil\xmark & \hfil\xmark  & \hfil\cmark & \hfil\xmark & \hfil\xmark & \hfil\cmark & \hfil\cmark & $k$  \\		%\ih{Does not belong here since it is local (supervised) DRE.}				
		
%		Bell et al.~\cite{Bell2013}	(STAR-Vote)	 & \hfil\cmark  & \hfil\xmark & \hfil\xmark & \hfil\xmark  & \hfil\cmark & \hfil\xmark & \hfil\cmark & ? & \hfil\cmark &  $k$  \\		%\ih{Does not belong here since it is local (supervised) DRE.}								
		
		%Juels et al.~\cite{juels2010coercion}		 & \hfil ? & ? & ? & ? & ? & ? & ? & ? & \hfil ? & \hfil ?  \\						
		
		Yu et al.~\cite{yu2018platform}	& \hfil\cmark & \hfil\cmark$^*$ & \hfil\cmark$^*$ & \hfil\cmark & \hfil\cmark$^*$ & \hfil\cmark & \hfil\cmark & \hfil\xmark  &  \hfil\xmark & \hfil $k$  \\						
				
		
		\textbf{BBB-Voting} & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark &  \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil\cmark & \hfil $k$\\
		
		\bottomrule
	\end{tabular}
	\vspace{5pt}
	\caption{A comparison of various remote voting protocols. $^*$Assuming a trusted $VA$.}
	\label{tab:comparison}
	\vspace{-0.8cm}
	%\zli{Please use black colour? }
\end{table*}


%Juels et al.~\cite{juels2010coercion} consider an adversary engaged in voter coercion -- in particular a demand to vote in an instructed manner.
% abstain or ask for voter decryption keys. 
%However, due to the remote nature of voting, their protocol remains susceptible to a pre-voting coercer present at that location. 
%In \name, the adversary is passive and our protocol is suitable for low coercion voting.   
%Chaum~\cite{chaum2004secret} introduces (Votegrity) a special type of voting receipt, which allows the voter to verify her vote at the voting booth, but safely encrypt the vote choice on the receipt before leaving the booth and yet verify her vote is included in the tally after leaving the booth. It is local voting.


%	\multicolumn{1}{c|}{}  Perfect ballot secrecy & Fair & Public verifiable & Self-tally & Fault-tolerant & Receipt-free & Scalable & Participant incentives & Continuous voting  \\


%\zli{There are various methods and approaches to electronic voting all around the world. %Each is connected with different benefits and issues. One of the most important and %prevalent problems is lack of auditing capabilities and system verification methods. }


%
%\zli{Sarad:
%While they are all e-voting protocols, blockchain specific implementation of two self-tallying protocols are discussed in McCorry et al.~\cite{McCorrySH17} and Li et al~\cite{Li2020}.}
%%However,
%%mention its shortcomings
%
%\zli{related works}
%
%
%
%
%
%Koens, Ramaekers and Wijk~\cite{ING:KoeRamWij17} provide a meaningful benchmark of zero-knowledge range proof (ZKRP) works, which can be used various applications, for example, voting.
%
%
%
%
%
%
%
%
%
%
%Kshetri and Voas~\cite{software:KshVoa18}
%
%
%Lopes, Pereira, and Varaj{\~{a}}o~\cite{AMCIS:LopPerVar19},
%
%
%
%
%
%
%
%
%
%
%Fusco~et~al.~\cite{IC3K:FLPP18} using secret sharing, but not very good.
%Moura and Gomes~\cite{DGO:MouGom17}, to short not necessary
%\href{http://scse.ntu.edu.sg/NewsnEvents/PublishingImages/SCSEFYP/Apr2019/FYPposters_x93_A1size_apr2019_set1_13.pdf}{blog}
%
%Hjalmarsson~et~al.~\cite{IEEECOUD:HHHH18},
%
%
%
%
%
%Hsiao~et~al.~\cite{CSA2:HTCW17}
%
%
%
%Panja~et~al.~\cite{EPRINT:PanRoy18}
%
%
%Bartolucci, Bernat, and Joseph~\cite{ICSE:BarBerJos18}
%
%
%Pawlak, Guziur and Poniszewska{-}Maranda~\cite{INCOS:PawGuzPon18}
%
%
%
%
%Hardwick~\cite{ithings:HGAM18},
%
%
%
%Hanifatunnisa and Rahardjo~\cite{TSSA:HanRah17}
%
%
%
%
%W{\"{u}}st and Gervais~\cite{CVCBT:WusGer18},






==> sec/security-analysis.tex <==
\vspace{-0.2cm}
In this section, we first analyze security of \name with regard to the voting properties specified in \autoref{sec:preliminaries}.
Next, we analyze blockchain-specific security \& privacy issues and discuss their mitigations. % \ih{while we compare some of them to the centralized e-voting}.
%
The security of our scheme relies on well-known cryptographic primitives under their standard assumptions.


%
%We base the privacy of votes in our protocol on ElGamal~\cite{Elgamal85} public-key cryptosystem.
%In detail, the ciphertext representing a blinded vote is a tuple ($c_1,c_2)$, where $c_1=g^{xy}.f$ and $c_2=g^y$, where the purpose of $c_2$ is to assist with the decryption.
%Decryption involves, computing $(c_2)^{-x}\cdot c_1$, to reveal $f$, which unambiguously identifies a vote choice. 
%These operations are carried out in a cyclic group.

\subsection{Properties of Voting}
\vspace{-0.3cm}
\par\noindent\textbf{(1) Privacy}
in \name requires at least 3 $P$s, out of which at least 2 are honest (see the proof in \autoref{sec:appendixvoteorivacy}).
Privacy in BBB-voting is achieved by blinding votes using ElGamal encryption~\cite{Elgamal85}, whose security is based on the decisional Diffie-Hellman assumption. Unlike the conventional ElGamal algorithm, a decryption operation is not required to unblind the votes. 
Instead, we rely on the self-tallying property of our voting protocol. 
%
The ciphertext representing a blinded vote is a tuple ($c_1,c_2)$, where $c_1=g^{xy}.f$ and $c_2=g^y$, where the purpose of $c_2$ is to assist with the decryption.
Decryption involves computing $(c_2)^{-x}\cdot c_1$ to reveal $f$, which unambiguously identifies a vote choice. 
%
As a result, the blinding operation for participant $P_i$ in \autoref{eqn:eq2} is equivalent to ElGamal encryption involving the computation of $c_1$ but not the decryption component $c_2$.
Furthermore, the blinding keys are ephemeral and used exactly once for encryption (i.e., blinding) of the vote within a single run of voting protocol 
-- i.e., if the protocol is executed correctly, there are no two votes $f_l$ and $f_m$ encrypted with the same ephemeral blinding key of $P_i$, such that 
\begin{equation}
 \frac{(g^{xy}\cdot f_l)} {(g^{xy}\cdot f_m)} = \frac{f_l}{f_m},  
\end{equation}
from which the individual votes could be deduced.  
For the blockchain-specific privacy analysis, see also (2) and (3) of \autoref{sec:blockchain-specific-issues}.




%\section{Security Analysis}
%\sarad{I feel we may omit the next sentence. ElGamal provides vote confidentiality but does not provide voter (identity) anonymity.} because no one can reveal the actual identity of the voter. Thus, ballot secrecy is held.

\par\noindent\textbf{(2) Ballot Secrecy.} It is achieved by blinding the vote using ElGamal homomorphic encryption~\cite{cgs97}, and it is not required to possess a private key to decrypt the tally because of the self-tallying property ($g^{\sum_{i}x_i y_i}=1$).
Therefore, given a homomorphic encryption function, it is possible to record a sequence of encrypted votes without being able to read the votes choices. 
However, if all $Ps$ are involved in the recovery of a partial tally consisting of a recorded set of votes, these votes can be unblinded (as allowed by ballot secrecy).
Even a subset of $n-2$ $P$s\footnote{Note that at least 2 $P$s are required to be honest (see \autoref{sec:adversary-model}).}  who have already cast their votes cannot recover a partial tally that reveals their vote choices because of the self-tallying property ($g^{\sum_{i}x_i y_i}=1$) has not been met. 
%As a result the blinding of the votes cannot be removed.
 
%Once all votes are cast, any involved party can perform the summation. %then the verification suite aggregates the local tallied votes.



%Generally, this homomorphic encryption is used to support self-tally.

%All that is required are the encrypted ballots themselves.

\par\noindent\textbf{(3) Fairness}. 
If implemented naively, the last voting $P$ can privately reveal the full tally by solving \autoref{eqn:eq3} before she casts her vote since all remaining blinded votes are already recorded on the blockchain (a.k.a., the last participant conundrum).
This can be resolved by $VA$ who is required to submit the final dummy vote including the proof of her vote choice, which is later subtracted from the final tally by $SC$.\footnote{Note that If $VA$ were for some reason not to execute this step, the fault recovery would exclude $VA$'s share from MPC keys, and the protocol would continue.}

%As shown in \autoref{eqn:eq1}, the participant's MPC key is a combination of ephemeral public keys from the all remaining participants, 

%which can guarantee fairness because the last participant conundrum is resolved by either $VA$ submitting the final dummy vote or by revealing its vote to a real candidate and having it removed from the tally.

\par\noindent\textbf{(4a) Universal Verifiability}. 
Any involved party can check whether all recorded votes in the blockchain are correct, and they are correctly included in the final tally~\cite{Kiayias2002}.
Besides, the blinded votes are verified at $SC$, which provides correctness of its execution and public verifiability, relying on the honest majority of the consensus power in the blockchain (see \autoref{sec:blockchain-specific-issues}).

%The blinded votes are verified at $SC$ using a witness indistinguishability proof of knowledge (see~\cite{Kiayias2002}), where a prover (i.e., $P$) demonstrates knowledge of the solution to some subset of given problem instances~\cite{CramerCrypto94}.
%%The verification of blinded votes presented in \autoref{fig:ZKPMultiCandidate} is based on the witness indistinguishability proof (see~\cite{Kiayias2002}).
%The verifier in \name is $SC$, which provides correctness of its execution and public verifiability, relying on the honest majority of the consensus power in the blockchain (see \autoref{sec:blockchain-specific-issues}).
%\ih{I am not sure about this witness indistinguishability proof.}
%The verification and announcement of tally result by $SC$ involves verifying that the the submitted tally fits \autoref{eqn:eq3}.

\par\noindent\textbf{(4b) E2E Verifiability}. 
To satisfy E2E verifiability~\cite{EPRINT:PanRoy18}, two properties should be met: 
(I) each $P$ can verify whether her vote was cast-as-intended and recorded-as-cast, 
(II) anyone can verify whether all votes are tallied-as-recorded.
\name meets (I) since each $P$ can locally compute her vote choice (anytime) and compare it against the one recorded in the blockchain.\footnote{Since $P$ can anytime (possibly upon coercion) create a receipt based on her vote choice (that cannot be changed), receipt-freeness is not provided.
% -- therefore, it is contradictory property to E2E verifiability. 
%Nevertheless, we argue that the receipt-freeness is a necessary property of the coercion resistance, which is in general not achieved in remote voting systems, such as \name and others. Besides, the coercion resistance (and thus receipt-freeness) are also not guaranteed even in local voting~\cite{chaum2008scantegrity}.
}
\name meets (II) since $SC$ executes the code verifying that the submitted tally fits \autoref{eqn:eq3} that embeds all recorded votes in the blockchain.

\par\noindent\textbf{(5) Dispute-Freeness}. 
Since the blockchain acts as a tamper-resistant bulletin board (see \autoref{sec:blockchain-specific-issues}), and moreover it provides correctness of code execution (i.e., on-chain execution of verification checks for votes, tally, and fault recovery shares) and verifiability, the election remains dispute-free under the standard blockchain assumptions about the honest majority and waiting the time to finality.


\par\noindent\textbf{(6) Self-Tallying}. 
\name meet this property since in the tally phase of our protocol (and anytime after), all cast votes are recorded in $SC$; therefore any party can use them to fit \autoref{eqn:eq3}, obtaining the final tally.

%\ih{Sarad, can you write sth, please?}
%\sarad{done. it was already there. moved some text around equation 2 here.}
%\ih{I think the following does not relate to self-tallying since self tallying only ensures that ``anybody can compute the tally after voting finishes''. I'd return it back to protocol.}
%$SC$ computes and stores the MPC key for each $P$ as follows:
%\begin{equation*}
%	\label{eqn:eqanakysis1}
%	\hspace{3cm} h=g^{y_i}=\prod\limits_{j=1}^{i-1} g^{x_j}/\prod\limits_{j=i+1}^{n} g^{x_j}, \hspace{3cm} (2)
%\end{equation*}
%where $y_i=\sum_{j<i}x_j- \sum_{j>i}x_j$
%and
%$\sum_{i}x_i y_i=0$ (see Hao et al.~\cite{HaoRZ10} for the proof).
%Since $y_i$ is derived from the private ephemeral keys of all other $P$s it is secret. % \ih{not relevant here}
%%
%While anyone can compute $g^{y_i}$, to reveal $y_i$ all $P$s $\setminus $ $P_i$ must either collude or solve the discrete log problem for \autoref{eqn:eq1}.\footnote{Note that this DLP was already computed for 795-bit long safe prime in 2019~\cite{integer-dlp-2019}; the computation took $\sim3100$ core-years, using Intel Xeon Gold 6130 (2.1GHz) CPUs.} 
%Since each $P_i$ can obtain $g^{y_i}$ of all $P$s, she alone can compute (ephemeral blinding key) $g^{x_i y_i}$ using her private key $x_i$.
%

\par\noindent\textbf{(7) Robustness (Fault Tolerance)}. 
%\ih{Sarad, can you write sth, please?}\sarad{done}
\name is robust since it enables to remove (even reoccurring) stalling $P$s by its fault recovery mechanism (see \autoref{sec:faulttolerance}).
Removing of stalling $P$s involves $SC$ verifiability of ZKP submitted by $P$s along their counter-party shares corresponding to stalling $P$s.
%
%Each pair of $P$s share exactly one slice of the ephemeral blinding key; this counter-party property is utilized in the fault recovery mechanism (see \autoref{sec:faulttolerance}).
%Only when all other participants combine, they are able to remove this slice of key belonging to the faulty participant, from each particiants' own encrypted vote. \ih{this is too detailed. Here is enough to justify that we support this property.}

\par\noindent\textbf{(8) Resistance to Serious Failures}. 
The resistance of \name to serious failures relies on the integrity and append-only features of the blockchain, which (under its assumptions \autoref{sec:blockchain-specific-issues}) does not allow the change of already cast votes. 

%\ih{Sarad, can you write sth, please?}
%\sarad{done.}
%Since a blockchain is a Byzantine fault tolerant state machine replication, it  tolerates a threshold number of serious failures that are adversarial and/or accidental in nature. 
%The consensus used in the blockchain (on which our voting protocol is implemented) will determine its exact tolerance to node and link failure in the presence of Byzantine faults. 

\subsection{Blockchain-Specific Aspects and Issues}\label{sec:blockchain-specific-issues}
\vspace{-0.3cm}
In the following, we focus on the most important blockchain-specific aspects and issues related to e-voting with \name.
For analysis of other potential issues and their comparison with centralized e-voting, we refer the reader to \autoref{sec:appendix-blockchain-vs-centralized-voting}, where we conclude that 
blockchain e-voting (with \name as the example) can only improve the potential problems of centralized e-voting (such as censorship, DoS, device exploitation) at the cost of more complex governance.

%In this section, we compare blockchain  e-voting with centralized e-voting since blockchain e-voting has received some critique~\cite{critic-blockchain-for-voting,park2021going} in the past. 



\par\noindent\textbf{(1) Bulletin Board vs. Blockchains}. 
The definition of a bulletin board~\cite{Kiayias2002} assumes its immutability and append-only feature, which can be provided by blockchains that moreover provide correct execution of code.
%While the bulletin board is a conceptual data structure, its expected behavior is not possible to perfectly guarantee neither in centralized voting nor blockchain voting.
%However, in centralized voting, a single entity can decide about removing/modifying an entry in the bulleting board, while in blockchain voting such a decision has to be made by a quorum of the honest majority. 
%Hence, the blockchain intuitively provides stronger append-only and immutability guarantees.


CAP theorem~\cite{brewer2000towards} enables a distributed system (such as the blockchain) to select either \textbf{\underline{c}}onsistency or  \textbf{\underline{a}}vailability during the time of network \textbf{\underline{p}}artitions.
If the system selects consistency (e.g., Algorand~\cite{gilad2017algorand}, BFT-based blockchains such as~\cite{hyperledger1}), it stalls during network partitions and does not provide liveness (i.e., the blocks are not produced) but provides safety (i.e., all nodes agree on the same blocks when some are produced). 
%
On the other hand, if the system selects availability (e.g., Bitcoin~\cite{Satoshi2009}, Ethereum~\cite{wood2014}), it does not provide safety but provides liveness, which translates into possibility of creating \textit{accidental forks} and eventually accepting one as valid.
%
Many public blockchains favor availability over consistency, and thus do not guarantee immediate immutability. 
%
%These accidental forks occur mainly due to a non-negligible network propagation delay, during which, several consensus nodes (i.e., miners) might produce different valid blocks at the same length, while only one of these blocks will be eventually included in a blockchain.\footnote{The winning block of such a fork contains a ``stronger'' value that meets the requested difficulty in contrast to losing block -- e.g., in Ethereum~\cite{wood2014} or Bitcoin~\cite{Satoshi2009}, where the stronger value of the target is represented by the smaller hash of a header. Note that in other consensus protocols (e.g., Algorand~\cite{gilad2017algorand}, HyperLedger~\cite{hyperledger1}), the notion of ``stronger'' is represented by the number of votes cast by the consensus nodes.} 
%
Furthermore, blockchains might suffer from \textit{malicious forks} that are longer than accidental forks and are expensive for the attacker. 
Usually, their goal is to execute double-spending or selfish mining~\cite{eyal2018majority}, violating the assumptions of the consensus protocol employed -- more than 51\% / 66\% of honest nodes presented in PoW / BFT-based protocols.
%\footnote{Note that the main goal of the selfish mining is to earn more than the fair ratio of the attacker's consensus power to the consensus power of the whole network; this is possible by letting other consensus nodes to waste their consensus power on building a chain that will be later replaced by a secret malicious chain.} 
%that require $33\%$ of the total consensus power or $51\%$ attacks that violate the assumptions of the consensus protocol employed within a blockchain but are the most expensive to execute. 
%
To prevent accidental forks and mitigate malicious forks in liveness-favoring blockchains, it is recommended to wait for a certain number of blocks (a.k.a., block confirmations / a time to finality). % which increases the probability that a transaction will remain irreversible after it appears in the blockchain. % and thus minimize the probability that the blockchain will be overridden -- such a time interval is referred to as \textit{a time to finality}. 
%For example, in Ethereum, the time to finality is equal to $\sim$3 minutes, which corresponds to 12 block confirmations.
%
Another option to cope with forks is to utilize blockchains favoring safety over liveness (such as~\cite{gilad2017algorand,hyperledger1}). % which provide immediate time to finality. % that is more convenient for the e-voting use case. 
%with a fast time to finalities, such as Algorand~\cite{gilad2017algorand}, HoneyBadgerBFT~\cite{miller2016honey}, or StrongChain~\cite{strongchain}. 
%

Considering \name, we argue that these forks are not critical for the proposed protocol since any transaction can be resubmitted if it is not included in the blockchain after a fork.
%
Waiting for the time to finality (with a potential resubmission) can be done as a background task of the client software at $P$s' devices, so $P$s do not have to wait.
Finally, we emphasize that the time to finality is negligible in contrast to timeouts of the protocol phases; therefore, there is enough time to make an automatic resubmission if needed.

\vspace{-0.1cm}
\par\noindent\textbf{(2) Privacy of Votes}. 
In \name, the privacy of vote choices can be ``violated'' only in the case of unanimous voting by all $P$s, assuming $\mathcal{A}$ who can link the identities of $P$s (approximated by their IP addresses) to their blockchain addresses by  passive monitoring of network traffic.
%
However, this is the acceptable property in the class of voting protocols that provide the full tally of votes at the output, such as \name and other protocols (e.g.,~\cite{McCorrySH17,Kiayias2002,HaoRZ10,killerprovotum,yu2018platform}).
%\footnote{Note that in the voting protocols with a \textit{tally-hiding} property~\cite{kusters2020ordinos,huber2022kryvos} that output only the winner, even unanimous voting should not reveal that it has happened.} 
%\ih{Sarad: do we have some examples of such protocols?}.
%\sarad{yes, there is a zero knowledge proof to determine if number a $>$ number b. We could do a logarithmic number of pairwise searches to determine which candidate has the largest number of votes without revealing their number of votes. however, there is some information leak because we can determine if $a<b$ for each of the ZKP output. Another option is to look at zero knowledge range proofs (see this https://arxiv.org/pdf/1907.06381.pdf). That can tell if $a\in [x,y]$ without revealing $a$. However, I dont know of any e-voting algo that does this. you might want to check. For unanimous voting too, i think you can do a range proof. but i dont see the point. The winning candidate has to be revealed finally. Hence, you know which candidate the unanimous (Single) voter had voted for.}
%
%\sarad{privacy of vote sounds vague. you may want to define it. above it sounds like data confidentiality, i.e., for which of $f_1,...f_k$ choices, the voter voted. Below it sounds like preventing linkage.}
%\ih{Privacy is defined in \autoref{sec:preliminaries}. And we do not have confidentiality defined in there -- I remember that we discussed that confidentiality is maybe a strong property, and we ended up with using the privacy only.}
Moreover, $\mathcal{A}$ can do deductions about the probability of selecting a particular vote choice by $P$s.
For example, in the case that the majority $m$ of all participants $n$ voted for a winning vote choice, then $\mathcal{A}$ passively monitoring the network traffic can link the blockchain addresses of $Ps$ to their identities (i.e., IP addresses), 
and thus $\mathcal{A}$ can infer that each $P$ from the group of all $P$s cast her vote to the winning choice with the probability equal to $\frac{m}{n} > 0.5$.
%\sarad{You could say... the blockchain stores only blinded votes. Hence a bijective map is not be established between the voter/candidate and their plain text vote.}\ih{this seems unrelated -- the point is that the final tally contains the majority of votes given to a single participant. So, $\mathcal{A}$ (that obtained mapping on its own by network monitoring) can infer that almost everybody voted for that participant, which I express by that probability.}
%
However, it does not violate the privacy of votes and such an inferring is not possible solely from the data publicly stored at the blockchain since it stores only blinded votes and blockchain addresses of $P$s, not the identities of $P$s.
To mitigate these issues, $P$s can use anonymization networks or VPN services for sending transactions to the blockchain. % precluding $\mathcal{A}$ from linking the blockchain addresses of $P$s with their identities.
%
Moreover, neither $\mathcal{A}$ nor $VA$ can provide the public with the indisputable proof that links $P$'s identity to her blockchain address since $P$s never provide $VA$ with such a proof (i.e., all communication of the identity verification is carried out without requiring $P$ to sign such a proof).
%All remaining communication is carried out through the blockchain.

\vspace{-0.1cm}
\par\noindent\textbf{(3) Privacy of Votes in Larger than Boardroom Voting}. 
%\myparagraph{\textbf{Mitigations}}
The privacy issue of unanimous and majority voting (assuming $\mathcal{A}$ with network monitoring capability) are less likely to occur in the larger voting than boardroom voting since the voting group of $P$s is larger and potentially more divergent.
We showed that \name can be extended to such a large voting by integrity-preserving batching in \autoref{ssec:scalability-improvements}. % where the number of $P$s is limited only by the expenses paid by $VA$ to register $P$s and compute their MPC keys.
We experimented with batching up to 1000 $P$s, which is a magnitude greater voting than the boardroom voting.
We depict the gas expenses paid by $VA$ (per $P$) in \autoref{fig:mpc-batches}, where we distinguish various batch sizes.
Results show that the bigger the batch size, the lower the price per~$P$.
%Such a batching mechanism imposes some overhead for preserving the integrity across batches; however, for all batch sizes, it was smaller than $1.0\%$ in contrast to disabled batching.




%\par\noindent\textbf{\textbf{Fault Recovery \& Adversary Controlling Multiple Participants.}}
%One issue that needs to be addressed in the fault recovery is $\mathcal{A}$ who controls multiple $P$s and let them stall one-by-one in each fault recovery round. 
%Even though the fault recovery mechanism will eventually finish with no new stalling $P$s, such a behavior might increase the costs payed by remaining $P$s who are required to submit counter-party shares in each round of the fault recovery.
%For this reason, similar to the voting stage, we require the fault recovery stage to penalize stalling $P$s by losing the deposit they put into $SC$ at the setup stage of our protocol.
%%
%%On the other hand, $\mathcal{A}$ can cause a certain delay of the whole protocol, which, however, should not be significant in the boardroom voting where most of the participants are expected to be on-line during the fault-recovery.
%%
%To further disincentivize $\mathcal{A}$ from such a behavior, the fault-recovery might require additional deposits that could be increased in each round by some constant.
%%Such deposits for the next round might be submitted to $SC$ within a fault recovery transaction of the current round, while all deposits could be redeemed at the tally stage.





==> sec/security.tex <==

The security of our scheme relies on well defined cryptographic primitives under their standard cryptographic assumptions.
ElGamal~\cite{Elgamal85} is the well studied public key cryptosystem on which we base the confidentiality of the votes in our basic protocol.
In ElGamal cryptosystem, the ciphertext is a two tuple ($c_1,c_2)$, where $c_1=g^{xy}.f$ and $c_2=g^y$. 
Decryption involves, computing the inverse of $(c_2)^x$ and multiplying it with $c_1$, to reveal $f$. 
These operations are carried out in a cyclic group.

\par\noindent\textbf{Confidentiality} is achieved by blinding the vote using ElGamal encryption, whose security is based on the decisional Diffie-Hellman assumption. Unlike the conventional ElGamal encryption, a per participant decryption operation is not required to unblind the tally (due to the self tallying property). Hence, the key material required for ElGamal decryption is not part of the blinded vote (ciphertext). I.e., we retain $c_1$ and discard $c_2$. 
As a result, the blinding operation for participant $P_i$ in \autoref{eqn:eq2} is equivalent to ElGamal encryption and inherits its security properties.
Further, the blinding keys are ephemeral, and used exactly once for encrypting (blinding) the vote.
I.e., if the protocol is correctly followed, there are no two votes $f_l$ and $f_m$ encrypted with a participants' same ephemeral blinding key, such that  $(g^{xy}\cdot f_l) / (g^{xy}\cdot f_m) = f_l/f_m$, from which the individual votes are deduced.  



%\section{Security Analysis}
%\sarad{I feel we may omit the next sentence. ElGamal provides vote confidentiality but do not provide voter (identity) anonymity.} because no one can reveal the actual identity of the voter. Thus, the ballot secrecy is held.

\par\noindent\textbf{Ballot secrecy} is achieved by blinding the vote using ElGamal homomorphic encryption~\cite{cgs97}, it is not required to possess a private key to decrypt the tally because of the self-tallying property ($g^{\sum_{i}x_i y_i}=1$).
In detail, the verification suite repeats on each booth (local) tally.
The reason is that given a homomorphic encryption function, it is possible to add a sequence of encrypted votes without being able to read the votes themselves. 
Once all votes are cast, any involved party can perform the summation themselves. %then the verification suite aggregates the local tallied votes.

%\IH{per each aggregated booth smart contract?} \sout{the smart contract-executed encrypted ballot aggregation.}



%Generally, this homomorphic encryption is used to support self-tally.

%All that is required are the encrypted ballots themselves.







\par\noindent\textbf{Fairness}. As shown in \autoref{eqn:eq1}, the participant's MPC key is a combination of ephemeral public keys from other participants, which can guarantee the fairness because the last participant conundrum is resolved by either the EA submitting the final vote to a dummy candidate or by revealing its vote to a real candidate and having it removed from the tally.

\par\noindent\textbf{Public verifiability and dispute-freeness}. Any involved party is able to check if all submitted votes are well formed and the final tally is correct.
This is achieved using a correctness proof on the vote and a blockchain for tamper-resistance.
The blinded votes are verified using a witness indistinguishability proof of knowledge, where a prover demonstrates knowledge of the solution to some subset of given problem instances~\cite{CramerCrypto94}.
The verification presented in \autoref{fig:ZKPMultiCandidate} is based on the witness indistinguishability proof in Kiayias et al.~\cite{Kiayias2002}.
Further, the blockchain acts as a tamper-resistant bulletin board.
Through a majority consensus, they agree to a unique view of the log (bulletin board) under its standard security assumptions.
As a result, they are assured that the results viewed on the logs are not tampered.
Since all steps in the protocol are verifiable and assured, the election remains dispute free.


%no participant (except for the last one) is able to learn about the outcome of the elections before the final result is published in our setting.

%Every vote and any partial tally, is encrypted using the public key of the tallying center.


\iffalse

\par\noindent\textbf{Receipt-freeness}.
The proposed receipt-freeness algorithm initiates two instances of the basic protocol (one each for real and fake vote).
As a result, the receipt-freeness relies on the security of the basic (ElGamal like) protocol in \autoref{ssec:basicprotocol}.

\par\noindent\textbf{Public verifiability}.
PVSS is for public verifiability of fault tolerance alone.
The security notion of PVSS is defined via the following game between a challenger and a probabilistic polynomial time (PPT) adversary $\mathcal{A}$. Both the adversary and the challenger $\mathcal{C}$ are given as input a security parameter $\lambda$.
\begin{compactenum}\setlength{\itemsep}{0pt}
 \item The challenger runs $Setup(\lambda)$ to obtain the set of public parameters along with the public keys and the secret keys of all the shareholders. Besides all the public keys, the adversary is also given the secret keys of $t-1$ corrupted shareholders.
 \item The challenger picks two random secrets $sk_0$ and $sk_1$ and a random bit $b\in \{0, 1\}$. Then he runs the distribution algorithm for the secret $t_b$ and sends all the resulting information to $\mathcal{A}$ along with $\{t_0, t_1\}$.
 \item The adversary $\mathcal{A}$ finally outputs a guess bit $b'\in\{0,1\}$ and wins the game if $b'=b$.
\end{compactenum}
We define the advantage of this static adversary $\mathcal{A}$, against a $(t, n)$-threshold PVSS as
$$\mathsf{Adv}_{PVSS}(\lambda)=|Pr[b=b']-1/2|,$$
where $\lambda$ is the security parameter.
Therefore, if for all adversaries $\mathcal{A}$, the probability of the adversary $\mathsf{Adv}_{PVSS}(\lambda)$ is a negligible function in $\lambda$, then we say that threshold-based PVSS scheme is secure against a static adversary.
For any static adversary $\mathcal{A}$ for the $(t, n)$-threshold PVSS scheme, there exists an algorithm that distinguishes the two distributions of the encryption and commitment schemes.
To prove the PVSS, the security reduction is to show that if there is an adversary $\mathcal{A}$ who can break our $(t,n)$-threshold PVSS then one obtains an algorithm to solve decisional Diffie-Hellman.
Further information is available in Schoenmakers~\cite{Schoenmakers99}.






\begin{theorem}
If the ElGamal is secure against indistinguishable chosen ciphertext attacks (IND-CPA), NIZK is computationally sound and zero-knowledge, PVSS is publicly verifiable, and there is a constant fraction $c$ of the voters ($0 < c \leq 1$) who check their latest submitted ballots w.r.t. the voter behaviour distribution D, then the proposed voting system is secure against static corruption.
\end{theorem}


\par\noindent\textbf{Sketched proof}. Below we sketched the proof by a series of games, in more detail:
\par\noindent\textbf{Game.0}. This is a factual game, here we assume the adversary owns a particular advantage (that he is willing to upper-bound) to win the game. The simulator answers the queries from the adversary depending on the specification of encryption.


\par\noindent\textbf{Game.1}.  This game is identical with the Game.0 except
that, in the voting phase, the voter's true choice is ignored and a random choice $\bot$ is chosen as the voter's input.
The adversary is trying to manipulate the vote on the voter's device without getting caught.
If we assume $0< c <1$ fraction of the voters check their latest submitted ballots, the probability of not getting caught when manipulating any single vote is $1-c$. In this case if the probability of being detected at least once is
\begin{eqnarray}
p=1-(1-c)^{\omega(\log{\lambda})}=1-negl(\lambda),
\end{eqnarray}
where $\omega(\log{\lambda})$ implies that the number of votes will be tampered for the security parameter $\lambda$. Thus, armed with the probability of
being detected $p$, there is no adversary can distinguish Game.1 from Game.0 with more than negligible probability.



\par\noindent\textbf{Game.2}. The current game is the same as Game.1 except that, in the tally phase, Game.2 does not use the secret key to decrypt the ciphertext of votes. Thus, Game.2 and Game.1 are indistinguishable.

\noindent
Hence, the probability of the adversary's advantage  $\mathsf{Adv}_{PVSS}(\lambda)$ in the final game is negligible. 

\fi

==> sec/securityrequiremets.tex <==

%\label{ssec:requirements}
A voting protocol is expected to meet a number of properties to be useful.
A list of such properties appearing in the works of Kiyayias et al.~\cite{Kiayias2002} and Groth~\cite{Groth2004} are given below.

%\begin{compactitem}
		\noindent\textbf{Confidentiality of the Vote:} A participant vote must not be revealed other than by using her decryption key or through a collusion of remaining participants in her voting group.
		%\IH{Please define here.}
		
		\noindent\textbf{Perfect ballot secrecy (PBS):} is an extension to confidentiality of the vote. 
		%\IH{confidentiality of the vote must be defined as the first -- reader does not know it. Also, confidentiality and privacy are different, and to me privacy looks more convenient.}.
		%Sarad: its confidentiality of vote, added above.
		It implies that a partial tally (finding partial results before voting ends) of votes is available, only if all remaining participants are involved in its recovery.	
		This constitutes the best case scenario for ballot secrecy, as remaining participants are required to remove their vote.	
				
		\noindent\textbf{Fairness:} implies that a tally may be calculated only after all participants have submitted their votes.
		%This is achieved by ensuring that the tally can be computed only after a timeout.(not true)
		
		\noindent\textbf{Verifiability:} means that any involved party can verify that all votes cast are legitimate and the final tally is correct.
		This is achieved by using a tamper-resistant, public bulletin board (in our case the blockchain) and zero knowledge proofs to verify well-formedness (validity) of submitted votes.
		
		
		\noindent\textbf{Self-tallying:} Once all the votes are cast, any involved party may compute the tally.
%		This property feeds into the public verifiability of the tally.
		Self-tallying systems need to deal with the fairness issues  because the last participant is able to compute the tally even before casting her vote.
		This is rectified with an additional verifiable dummy vote~\cite{Kiayias2002}.
		%\IH{put some reference that proposes it}.
		%Another solution is to enforce that participants first commit their votes within a timeout.
		%Although the last participant is still able to compute the final tally before anyone else does, she is no longer able to change her vote.
						
		\noindent\textbf{Dispute-Freeness:} extends the notion of verifiability.
		All votes and the tally can be verified by any involved party to be correct, hence, the result is indisputable.
		%For the elections to be dispute-free, all disputes need to be resolved prior to its tally.
		%Note that dispute-freeness is not the same as dispute-resolution. % maybe DROP
		
		
		\noindent\textbf{Fault Tolerance (Robustness):} The voting protocol is able to recover from a fixed number of faulty participants. I.e., the protocol removes participants who may quit just before the voting step or attempt to vote incorrectly.
		%Non-conforming participants are removed by the protocol without affecting the votes of the remaining participants.
			
		%\noindent\textbf{Receipt-Freeness:} A participant is unable to supply a receipt of her vote after casting the vote.
		%The goal of receipt-freeness is to prevent vote selling.
		%This property also prevents a post election coercion~\cite{Benaloh1994,Hirt2000}, where a participant may be coerced to reveal her vote.
		%For example, receipt-freeness is a pre-condition for large centralized elections (e.g. national elections).
		%In a distributed setting, receipt-freeness requires an authority to supply additional entropy to the participants (see \autoref{ssec:receiptfreeness}).
		
	
		%\noindent\textbf{Receipt-indistinguishability:}
		%We define the weaker notion of receipt- indistinguishability aimed at reducing coercion.
		%Receipts of a participants' real and fake votes are available to a post election coercer, but are indistinguishable to the coercer with a tunable probability. 
		%\IH{Please define here.}
	
%\end{compactitem}


==> sec/unlinkability.tex <==


%In a practical scenario, only a subset of booth participants may be available to vote at any given epoch.
%This allows an attacker to identify non-voters.
In our model, we assume an adversary is able to run sybil nodes~\cite{chainalysis2015} on the blockchain network, read transactions passing through it and capture participant IP addresses.
%We have not so far attempted to break the map between participant wallet address and their actions on the blockchain across different tally cycles.
A mitigation to thwart attacks from sybil nodes is to use virtual private networks and mixnets.
However, anyone may parse the blockchain ledger for transactions generated by a participant wallet address and map it to her activity across various election epochs.
The work in Groth \cite{Groth2004} proposed a shuffle solution to break the map between a participant and their vote. 
Lai et al.~\cite{Lai2018} used stealth addresses to encode the candidate choice in the public key but their objective was to obfuscate participant vote.
In our scheme, we use wallet addresses to keep track of authorized participants.
In this section, we \textbf{propose an algorithm to break the map} between a participant and her wallet address by generating a new address for every epoch a participant wishes to vote.
The wallet address is generated as a function $f$ of the elliptic curve public key (e.g., a bitcoin wallet address~\cite{bitcoinaddress2019}). 
I.e., once the public key is available, it is straightforward for anyone to compute the corresponding wallet address.

The objective is to synchronize a practically unlimited number of wallet public keys (up to one per epoch) between $EA$ and a participant $P_i$ such that this public key list can be regenerated only by these two parties and the corresponding private keys can be regenerated only by $P_i$.
%While the public key at any future epoch can be regenerated by both $EA$ and $P_i$ (without extra storage requirements), the corresponding private key is known only to $P_i$. 
%At the start of each epoch where a participant wishes to vote, a new wallet address is generated by the participant and send to the smart contract.
%This address is validated for eligibility by $EA$, who then proceeds to set the state of new address on the smart contract to valid/invalid. 
%To simplify wallet management and synchronization between $EA$ and participant, we use a  cryptographically secure pseudo random number generator (CSPRNG) and a keyed hash.
The core idea behind the solution presented here is based on type 2 deterministic wallets (see \cite{deterministicwallet2019,Maxwell2011}).
Let $BP$ be the base point on the elliptic curve.
Further, let $PK$ be the public key corresponding to a secret key $SK$.
Here, $SK$ is chosen as a random positive integer whose size is bounded to the order of $BP$ on the chosen elliptic curve modulo a prime number. 
Note these keys are different from the ephemeral keypair used to blind the vote.
This discussion relates to wallet private and public keys.
As an illustration, let the first public key be computed as, $A0_{PK} = A0_{SK}\cdot BP$
and the next public key, 
$A1_{PK} = A0_{PK}+A1_{SK}\cdot BP$.
%Also, 
%$A1_{SK} = A0_{SK}+A1_{SK}$.
Here, we observe that $(A0_{SK}+A1_{SK})\cdot BP = A0_{SK}\cdot BP +A1_{SK}\cdot BP = A0_{PK} + A1_{SK}\cdot BP = A1_{PK}$.
The following steps ensue:
\begin{compactenum}
	\item Participant $P_i$ at identify verification step, in additional to her wallet address $W_{i,0}$, deposits with the $EA$ both wallet public key $PK_{i,0}$, a shared secret key $hk_i$ and CSPRNG parameters (e.g. Chacha20~\cite{chacha20}).
	
	\item The private key of $P_i$ at any future epoch $e$  is generated by $P_i$ as   
	$SK_{i,e}= SK_{i,0} + $HMAC$_{hk_i}(CSPRNG_e)$.
	Here, $CSPRNG_e$ is the output of pseudo random number at epoch $e$, HMAC$_{hk_i}(.)$ is a hash-based message authentication code using shared secret key ${hk_i}$.
	
	\item The corresponding public key of $P_i$ is   
	$PK_{i,e}= PK_{i,0} +$ HMAC$_{hk_i} (CSPRNG_e)\cdot BP$.
	The public key can be computed by $EA$ and $P_i$ but all private keys are computable only by $P_i$.
	This effectively separates out the PK's from their SK's and at the same time chains it to $P_i$'s first wallet public key, i.e. $PK_{i,0}$.   
	
\end{compactenum} 

At any epoch $e$, the public key $PK_{i,e}$ and the corresponding wallet address can be computed by both $EA$ and $P_i$.
Since the shared secret $hk_i$ used with HMAC is known only to $EA$ and $P_i$, no third party is able to compute any future public keys. Since wallet address of $P_i$, $W_{i,e}$ = $func(PK_{i,e})$, the map between the wallet address and the participant is broken for all other parties other than $EA$ and $P_i$.
Note the above operations are computed offline.
The $EA$ merely sets a valid/invalid flag on the smart contract for the new wallet address posted there by $P_i$.
Since an adversary is no longer able to infer identity of wallet addresses to writes on the blockchain ledger, it prevents further statistical inference attacks.
The additional requirement for this modification to work is that $EA$ is trusted to carry out the above operations honestly.
Alternately, $EA$ may be replaced by a group of notaries to improve trust.

